Program Targeting with Machine Learning and Mobile Phone Data: Evidence from an Anti-Poverty Intervention in Afghanistan

Can mobile phone data improve program targeting? By combining rich survey data from a "big push" anti-poverty program in Afghanistan with detailed mobile phone logs from program beneficiaries, we study the extent to which machine learning methods can accurately differentiate ultra-poor households eligible for program benefits from ineligible households. We show that machine learning methods leveraging mobile phone data can identify ultra-poor households nearly as accurately as survey-based measures of consumption and wealth; and that combining survey-based measures with mobile phone data produces classifications more accurate than those based on a single data source.

==> Targeting Paper_COPY2/abstract.tex <==
% ------- COVID-y abstract -------%

%As COVID-19 spreads in low and middle-income countries, economic disruptions have left hundreds of millions without work or income.  To offset the pandemic’s most devastating effects, national policymakers and humanitarian organizations are scrambling to distribute emergency assistance to those who need it most. However, many countries lack reliable and up-to-date information about on-the-ground economic conditions, and have no way of collecting these data in the middle of a pandemic.

%This paper uses rich data from Afghanistan to ask the question: Can machine learning, as applied to vast repositories of mobile phone data, be used to accurately identify the most poor and vulnerable households? We combine household survey data from a ``big push'' anti-poverty program in Afghanistan with detailed logs of mobile phone activity from the country's largest mobile phone operator, and test the accuracy of machine learning algorithms in differentiating between ultra-poor households eligible for program benefits and other poor households that are ineligible. We show that the algorithmic approach can identify ultra-poor households as accurately as standard survey-based measures of poverty, including consumption and wealth; and that combining survey-based measures with mobile phone data produces classifications more accurate than those based on a single data source.

%\textit{Note to MD4SG committee:} The analysis in this manuscript is based on historical data from Afghanistan. Since April 2020, we have been working with the government of Togo to implement this ML approach to target emergency COVID-19 aid in the country - see \cite{blumenstock2020}. These results are not described in the working paper, but preliminary results will be ready for presentation in August.

%\textit{Note to NBER Economics of AI committee:} The analysis in this manuscript is based on historical data from Afghanistan. Since April 2020, we have been working with the government of Togo to implement this ML approach to target emergency COVID-19 aid in the country - see \cite{blumenstock2020}. These results are not described in the working paper, but will be ready for presentation in September.


% ------- Non-covid Abstract ------%

%Can non-traditional data be used to more efficiently target development aid? By combining rich survey data from a ``big push'' anti-poverty program in Afghanistan with detailed mobile phone logs from program beneficiaries, we study the extent to which machine learning methods can accurately differentiate ultra-poor households eligible for program benefits from ineligible households. We show that supervised learning methods leveraging mobile phone data can identify ultra-poor households as accurately as standard survey-based measures of poverty, including consumption and a proxy of wealth; and that combining survey-based measures with mobile phone data produces classifications more accurate than those based on a single data source. 

Can mobile phone data improve program targeting? By combining rich survey data from a ``big push'' anti-poverty program in Afghanistan with detailed mobile phone logs from program beneficiaries, we study the extent to which machine learning methods can accurately differentiate ultra-poor households eligible for program benefits from ineligible households. We show that machine learning methods leveraging mobile phone data can identify ultra-poor households nearly as accurately as survey-based measures of consumption and wealth; and that combining survey-based measures with mobile phone data produces classifications more accurate than those based on a single data source. 

==> Targeting Paper_COPY2/discussion.tex <==
Our key finding is that, in a sample of 535 phone-owning households in poor villages in Afghanistan, machine learning methods leveraging phone data are nearly as accurate at identifying ultra-poor households as standard asset- and consumption-based methods. Further, we find that methods combining survey data with CDR perform better than methods using a single data source.  However, as we demonstrate empirically, low rates of phone ownership --- or the inability to access data from all operators --- can undermine the value of CDR-based targeting. In our setting, the CDR-based approach still works well if households without phones are targeted before the CDR-based algorithm selects the poorest households with phones. However, this approach may not be appropriate in other contexts where phone ownership is less predictive of wealth, or where potential beneficiaries have the ability to strategically under-report phone ownership \citep{bjorkegren2020manipulation}.

As mobile phone penetration rates continue to rise in LMICs \citep{gsma}, and as programs increasingly rely on mobile phones and money to distribute benefits \citep[cf.][]{gentilini_social_2020}, CDR-based targeting methods will likely play a more prominent role in the set of options considered by policymakers and program administrators --- particularly in contexts like Afghanistan, where traditional targeting benchmarks are missing or of low quality. In just the past few years, for instance, data from mobile phone operators was used in the design of social assistance programs in Colombia, the Democratic Republic of the Congo, Pakistan, and Togo \citep{gentilini_social_2020,gentilini2021cash,aiken_machine_2021}. We conclude by highlighting a few policy important considerations for CDR-based targeting.

\paragraph{Speed and cost} An advantage of CDR-based targeting is that it can be used in contexts where face-to-face contact is not feasible, dramatically reducing the time required to implement a targeted  program. While it typically takes many months (or years) to implement a proxy-means test (PMT), community-based targeting (CBT), or consumption-based targeting, a CDR-based model can be trained in just a few weeks (see Appendix \ref{sec:appendix:costs}). Likewise, the marginal costs per household screened are substantially lower with CDR-based targeting than with CBT, PMT, or consumption-based targeting. For instance, Table \ref{appendix:costs} uses cost estimates obtained from the literature (and detailed in Table \ref{appendix:costliterature}) to estimate targeting costs for the TUP program.\footnote{In our cost calculations we obtain estimates for a CBT, rather than the hybrid approach used in the TUP program, as there is more information available on CBT-only costs in the literature. However, as the CBT cost can be interpreted as a lower bound for the cost of a hybrid approach, our qualitative results also apply to a hybrid approach.}  Whereas the marginal costs of screening an individual with a CBT or PMT are estimated at \$2.20 and \$4.00, respectively, the marginal cost of screening with CDR is negligible (see Appendix \ref{sec:appendix:costs}).\footnote{Marginal costs of CDR-based targeting are negligible because we assume no contact with screened individuals is required. In practice, it may be desirable to solicit informed consent to access CDR. If consent were collected in-person, the marginal costs would approach that of a PMT; if collected over the phone,  there would still be significant cost savings, see Appendix Section \ref{sec:appendix:costs}).}
For the entire TUP program, which screened around 125,721 households in six provinces, CBT and PMT would add an additional estimated \$276,586 and \$502,884, respectively, corresponding to 2.18\% and 3.97\% of the total program budget. 

\paragraph{Data access and privacy} Access to phone data is necessary for CDR-based targeting. As we show, targeting performance degrades considerably when CDR are not available for subsets of the population. Encouragingly, the past several years have been characterized by a trend towards public sector access to CDR, particularly in the context of the COVID-19 pandemic, during which mobile network operators shared CDR with governments, researchers, and NGOs for social protection purposes \citep[cf.][]{gentilini_social_2020,gentilini2021cash,aiken_machine_2021}. CDR have also been shared with the public sector for public health and humanitarian aid applications \citep{milusheva2021challenges}. Access issues aside, CDR contain private and sensitive data, including phone numbers and location traces. While much has been written about enabling responsible use of CDR for humanitarian response \citep[e.g.][]{de2018privacy,oliver2020mobile}, to date no consistent privacy standards exist. Informed consent can increase participant agency, but also complicates the implementation logistics. Likewise, there may be ways to incorporate differential privacy or other privacy enhancing technologies into a CDR-based targeting system, but such privatization would likely decrease targeting accuracy \citep{hu2015differential}.

% These results extend past work on wealth estimation from mobile phone data to suggest that CDR methods --- and perhaps methods using other sources of digital trace data --- could be used in practice to target anti-poverty programs or other development interventions. Moreover, reviews of standard field-based poverty targeting schemes find that targeting is limited by low-quality ground truth data on well-being benchmarks across programs and regions \citep{brown2018, coady2004}. CDR-based methods like the one presented here could provide a lower-cost complement to standard targeting methods without sacrificing accuracy, and would be particularly useful in unstable or conflict-affected regions where field-based targeting is not viable.

%However, as we demonstrate empirically, low rates of phone ownership --- or the inability to access data from all operators --- can undermine the value of CDR-based targeting. While mobile phone penetration rates continue to rise in LMICs \citep{gsma}, we expect that, for the forseeable future, CDR-based methods may be best deployed in conjunction with alternative approaches.  In our specific setting, the CDR-based approach still works well if households without phones are targeted before the CDR-based algorithm then selects the poorest households with phones. However, this approach may not be appropriate in other contexts where phone ownership is less predictive of wealth, or where potential beneficiaries have the ability to strategically under-report phone ownership \citep{bjorkegren2020manipulation}.

% We emphasize, however, that CDR-based targeting applies only to households that own a mobile phone, so CDR-based methods are inherently limited by mobile phone penetration rates. We therefore simulate, using population-representative data from the TUP survey, targeting with CDR under conditions of limited household phone penetration. We find that CDR-based targeting is not useful under conditions of low household phone  ownership, but maintains its accuracy when phones are prevalent but not ubiquitous, particularly when all non-phone-owning households are made program-eligible.

% The 535-household subsample analyzed above make up only 19\% of the 2,814 households surveyed in the TUP program. Households are left out of the subsample for one of several reasons: they may not own a phone, they may own a phone that is not on the mobile network for which we observe CDR (this network is estimated to have around 30\% market share in Afghanistan), or they may own a phone that was not active during the six months of CDR data collection. Therefore, it is not inconsistent that while only 19\% of the households in the TUP survey are matched to CDR in our analysis, 84\% of the households report owning at least one mobile phone.

%As mobile phone penetration rates continue to rise in LMICs \citep{gsma}, CDR-based methods will become increasingly relevant, but an understanding of the distribution of mobile phone ownership among the poor and very poor is essential to practical deployment of the methods introduced here. Given this limitation and our promising results on combining CDR with standard targeting measures for increased classification accuracy, CDR-based methods may be best deployed in conjunction with standard targeting methods so that survey-based data is complemented by digital trace data. Moreover, the methods for targeting non-phone-owners simulated here -- namely blanket targeting non-phone-owners or blanket eligibility for non-phone-owners -- are appealing in their simplicity but are not the only approaches to addressing incomplete phone ownership for CDR-based targeting. One alternative is allowing non-phone-owners to register for programs by borrowing another's phone -- though this strategy raises questions of homophily and phone sharing that could only be addressed with an empirical study.

% Our analysis also highlights several broader considerations that merit deeper investigation in future work. These include:
% In addition to the issue of incomplete phone ownership, there are ethical trade-offs specific to targeting with CDR and other non-traditional data sources. 


%Beyond individual autonomy, regulatory barriers may impede access to CDR, and moreover if bad actors gain access, CDR could be used to target subscribers for interventions far less desirable than aid. Formal privacy guarantees could help ensure that CDR cannot be misused \citep{hu2015differential}, but there is an inherent trade-off between privacy and data utility when statistical privacy guarantees are introduced. 

\paragraph{Algorithmic transparency and strategic behavior} Using CDR to determine program eligibility may introduce incentives for people to manipulate their phone use. This consideration is not unique to CDR, as degrees of manipulation have been documented in social programs that use proxy means tests and other traditional targeting mechanisms \citep{camacho_manipulation_2011,banerjee_lack_2018}. Indeed, complex and non-linear machine learning algorithms, like the one presented in this paper, may obfuscate the logic behind targeting decisions, reducing the scope for manipulation. However, society often demands transparency in algorithmic decision-making, as black-box decisions are difficult to audit or hold to account. There is therefore a tension between the goals of increasing transparency and reducing manipulation, though recent advances in machine learning explore mechanisms for pursuing both objectives at once \citep{bjorkegren2020manipulation}.

% Several studies have documented that, when potentially eligible beneficiaries are made partially or fully aware of the decision rule used in targeting mechanisms, a subset of beneficiaries are likely to manipulate their observable characteristics to become program-eligible. Mobile phone data is likely to be no exception, especially in the case of blanket targeting based on mobile phone ownership. One solution to the problem of strategic behavior is to use black-box machine learning algorithms, like the one presented in this paper, to make targeting decisions. Since the decision rule is not easily explainable to potential beneficiaries or other stakeholders, manipulation of eligibility is challenging.  On the other hand, black-box decisions make auditing algorithmic integrity difficult, and offer little recourse for correcting inevitable targeting mistakes.

\paragraph{Centralized vs. local knowledge} CDR-based methods enable a top-down, centralized and standardized approach to program targeting, rather than a bottom-up approach that prioritizes local knowledge that can be elicited, for example, through community wealth rankings. While the empirical results in this paper indicate that the efficiency gains from CDR-based targeting are substantial, it may reinforce existing power structures \citep{taylor,blumenstockbigdata,abebe_narratives_2021}. Efficiency gains should also be considered within the context of evidence suggesting that participating communities may prefer community-based approaches \citep{alatas2012}, but also may perceive them as less legitimate \citep{Premandetal2020}. 


\paragraph{} To summarize, our results suggest that there is potential for using CDR-based methods to determine eligibility for economic aid or interventions, substantially reducing program targeting overhead and costs. Our results also indicate that CDR-based methods may complement and enhance existing survey-based methods. We note, however, that the practical and ethical limitations to CDR-based targeting are significant. We emphasize the need to consider these limitations and the constraints of specific local contexts alongside the efficiency gains offered by CDR-based targeting.


%As a secondary finding, we note that in contrast to the relative success of CDR-based methods for identifying the ultra-poor in this sample, our CDR-based methods have little predictive power for estimating an asset-based wealth index or consumption among the TUP households. We hypothesize that there may be aspects of the ultra-poor classification that make it easier to estimate than other wealth measures. Recall that ultra-poor classification in our sample is based on a community wealth ranking followed by verification of qualifying criteria that cover several aspects of poverty and deprivation. It is possible that ultra-poor status is simply a less noisy than the other ground-truth wealth measures: it is based on  multiple components, which helps reduce measurement error, and qualifying criteria were validated in-person by ministry staff, which adds an element of objectivity. An alternative hypothesis is that the ultra-poor are a segment of the population that is easier to identify through behavioral traces in mobile phone data. \cite{alatas2012} suggest that communities apply a concept of wealth beyond income, consumption, or assets in their wealth rankings; it could be that this concept is better reflected in mobile phone traces than the standard quantified welfare measures. Further, the additional qualifying criteria for ultra-poor status cover heterogeneous aspects of welfare relating to income, housing, assets, and education. It is possible that this holistic measure of wealth is better reflected in the digital footprint of the ultra-poor than specific asset or consumption-based indicators.

%We also present several hypotheses for why the prior success of CDR-based wealth index prediction methods \citep{blumenstock2018, blumenstock2015} does not replicate to the sample we analyze. First, machine learning methods perform better with large amounts of training data, and the sample size of this dataset (537 households) is significantly smaller than the samples used in previous CDR work, which include datasets from Rwanda with 856 individuals \citep{blumenstock2015} and Afghanistan with 1,234 households \citep{blumenstock2018}. Second, the components used to construct wealth indices vary between wealth prediction projects, and it is possible that the wealth index used here is less useful (or less predictable) than those used in past work. Although early papers indicate that asset-based wealth indices are robust to changes in the underlying set of components \citep{filmer2001, wagstaff}, subsequent work has found that household wealth categorization can be sensitive to the assets selected for inclusion \citep{houweling, michaelson}. Third, it may be that structural differences between the type of sample we analyze here and those used in previous work can account for differences in predictive power. Most significantly, the sample of households here is drawn from poor villages in a single rural province of Afghanistan, whereas previous samples have included households across the socioeconomic spectrum from several or all provinces in a country. We hypothesize that much of the variation picked up by CDR-based models in previous work captures stark rich-poor inequalities and urban-rural divides; it may be much more challenging to train models that pick up on variation in a relatively homogeneous sample of poor households using CDR data. This hypothesis is consistent with previous work showing that distinguishing between the very wealthy and the very poor is easier than discerning finer variations in welfare, even with standard survey-based measures of wealth \citep{karlan2013}.

%Our results suggest that there is potential for using CDR-based methods to target vulnerable members of society for economic aid or interventions, significantly reducing program targeting overhead and costs. Our results also provide evidence that CDR-based methods could complement and enhance existing survey-based methods for better targeting accuracy.  However, we emphasize that, as demonstrated by their low predictive power for wealth and consumption in our sample, CDR-based methods are not one-size-fits-all and cannot be blindly adapted to new contexts without careful tuning and validation. There is much room for future work demonstrating the use of CDR-based wealth prediction and targeting in new contexts to build the literature on when and how these methods can be effectively and appropriately leveraged for policymaking.



==> Targeting Paper_COPY2/intro.tex <==
% JB: I moved the old intro into "intro_new.tex" in case people prefer the prior version

Each year, hundreds of billions of dollars are spent on targeted social protection programs. The importance of these programs increased dramatically in the past 18 months: In 2020, global extreme poverty increased for the first time in two decades, and most countries expanded their social protection programs, with more than 1.1 billion new recipients receiving government-led social assistance payments \citep{gentilini_social_2020}. 

Determining who should be eligible for program benefits --- \textit{targeting} --- is a central challenge in the design of these programs \citep{hannaolken,lindert2020sourcebook}. In high-income countries, targeting frequently relies on tax records or other administrative data on income. In low- and middle-income countries (LMICs), where a large fraction of the workforce is informal, programs often require primary data collection. The difficulty and cost of collecting data, and the variable quality of what gets collected, can introduce significant errors in the targeting process \citep{Deaton2016,jerven, wb_forthcoming}. These issues are exacerbated in fragile and conflict-affected countries, where two thirds of the world's poor are expected to reside by 2030 \citep{corral2020}. 
% Consumption and poverty estimates are based on surveys with quality issues, and ``in some cases, the problems are severe enough to threaten even the most basic understanding of growth, poverty and inequality" \citep{Deaton2016}.}

This paper evaluates the extent to which non-traditional administrative data, processed with machine learning, can be used for program targeting. Specifically, we match call detail records (CDR) from a large mobile phone operator in Afghanistan to household survey data from the Afghan government's Targeting the Ultra-Poor (TUP) anti-poverty program. Eligibility for the TUP program was determined through a \textit{hybrid targeting method}, combining  a community wealth ranking (CWR) and a short follow-up survey. We then assess the accuracy of three counterfactual targeting approaches at identifying the actual beneficiaries of the TUP program: (i) our \textit{CDR-based method}, which applies machine learning to data from the mobile phone company; (ii) an \textit{asset-based wealth index}, which uses asset ownership to approximate poverty; and (iii) \textit{consumption}, a common benchmark for measuring poverty in LMICs.

Our analysis produces three main results. First, by comparing errors of inclusion and exclusion using the program's hybrid method as a benchmark, we find that the CDR-based method is nearly as accurate as the commonly-employed asset and consumption-based methods for identifying the phone-owning ultra-poor households. Second, we find that methods combining CDR data with measures of assets and consumption are  more accurate than methods using any single data source. Third, we find that when non-phone-owning households are included in the analysis, the CDR-based method remains accurate if non-phone-owning households are classified as ultra-poor; however, targeting performance is quite poor if households without phones are ineligible for benefits. After presenting these main results, we compile data from several existing targeting programs to give an indication of the substantial reduction in marginal costs associated with CDR-based targeting.

These results connect two distinct strands of prior work. The first is a literature on program targeting, which studies the effectiveness of different mechanisms for identifying program beneficiaries. In LMICs, research has focused on the performance of proxy means tests (PMTs) \citep{grosh1995proxy,filmer2001,brown2018}, community-based targeting strategies (CBTs) \citep{alatas2012,Fortinetal2016}, and related approaches \citep{banerjee2007,karlan2013,Premandetal2020}. A meta-analysis by \citet{coady2004}, which includes 8 PMTs and 14 community-based programs, finds little difference in targeting accuracy between the two methods --- but notes that targeting is regressive in a quarter of programs reviewed. In addition to issues with targeting accuracy, the current methods available for poverty targeting in LMICs are time- and resource-intensive, and  may be infeasible in fragile or conflict-affected areas or in contexts where social interaction is limited, such as during a pandemic. 

% While \textit{per capita} consumption is often used as a benchmark to estimate poverty and measure targeting errors, the evidence comparing PMT and community-based approaches suggests that communities may apply a broader concept of poverty---for instance, including factors that predict earnings capacity. Community-based methods also typically yield higher rates of community satisfaction levels than PMT methods, when elite capture is absent. \citep{alatas2012,banerjee2007,Fortinetal2016,karlan2013,Premandetal2020}.\footnote{Contrary to this evidence, a study in Cameroon finds that community-based targeting methods performed consistently worse compared to PMT selection when assessed against consumption. However, the authors explained, that these are in part driven by communities including human and physical capital asset holding in the selection criteria---consistent with a multidimensional concept of poverty---and also due to implementation issues, reflected in errors of exclusion and inclusion above 40\% for PMT \citep{Stoeffler2016}}.

The second body of work explores the extent to which non-traditional sources of data, in conjunction with machine learning, might help address data gaps in LMICs  \citep[e.g.,][]{blumenstock2016,burke2021}. Much of this work focuses on estimating the geographic distribution of poverty at fine spatial granularity, using data from satellites \citep{jean_combining_2016,engstrom2017poverty}, mobile phones \citep{blumenstock2015,hernandez}, social media \citep{fatehkia2020mapping,ermon2019}, or some combination of these data sources \citep{steele2017,pokhriyal,chi_micro-estimates_2020}.
% \footnote{This body of work focuses largely on poverty, typically quantified by an asset-based wealth index \citep[e.g.][]{blumenstock2015, hernandez}, but related papers explore a wider set of well-being measures, including literacy \citep{schmid}, food security \citep{decuyper1}, and infrastructure \citep{blumenstock2017}.}
Most relevant to our current analysis, two prior papers investigate whether the mobile phone use can approximate the wealth of individual mobile subscribers. \cite{blumenstock2015} show that CDR data are predictive of an individual-level asset-based wealth index among a nationally representative sample of 856 Rwandan mobile phone owners ($r$ = 0.68).  \cite{blumenstock2018} finds similar results with a sample of 1,234 male heads of households in the Kabul and Parwan districts of Afghanistan. While these results show that phone data can be used to \textit{predict} poverty levels, they do not evaluate whether those poverty estimates are of sufficient quality for real-world policy applications. 

Our paper connects these two literatures by rigorously assessing the extent to which phone-based estimates of poverty can help with program targeting \citep{blumenstock2020}.
We believe the analysis will be especially relevant to the increasing number of interventions that rely on mobile money to distribute cash payments \citep{gentilini_social_2020}, and the growing number of contexts where mobile phone data are being made available for humanitarian purposes \citep{milusheva2021challenges}. For example, in just the past few years, mobile money was used to make cash transfer payments in countries including Bangladesh \citep{mm_bangladesh}, Ghana \citep{mm_ghana}, Liberia \citep{mm_liberia}, and Malawi \citep{mm_malawi}. Mobile phone \textit{data} has been used to guide cash transfers in Colombia \citep{gentilini_social_2020}, the Democratic Republic of the Congo \citep{gentilini2021cash}, Pakistan \citep{gentilini_social_2020}, and Togo \citep{aiken_machine_2021}.%
\footnote{The anti-poverty program implemented in Togo and described by \citet{aiken_machine_2021} was based on the methods developed and evaluated in this paper. Due to the time-sensitive nature of the COVID-19 response described in \citet{aiken_machine_2021}, the two academic articles are in circulation concurrently.}

The context of our empirical analysis -- identifying ultra-poor households in Afghanistan -- is a particularly challenging environment for data collection and program targeting, as 62\% of the households classified as not \textit{ultra}-poor still fall below the national poverty line. In such environments, when traditional options for targeting are not feasible, these methods may provide a viable alternative for identifying households with the greatest need. Given the policy relevance of these results, we conclude our analysis by discussing important ethical and logistical considerations that may influence how CDR methods are used to support targeting efforts in practice.


%The two manuscripts also have distinct foci: \citet{aiken_machine_2021} documents the performance of a CDR-targeted anti-poverty program in rural Togo, with in-depth results on exclusions caused by practical aspects of the implemented program; our paper documents the strengths and weaknesses of a CDR-based approach to targeting the ultra-poor in Afghanistan, and provides novel results on the benefits of combining CDR with other data, and considerations regarding households without phones.}

%recent breakthroughs in mobile phone data access for social protection and humanitarian purposes \citep{milusheva2021challenges} make phone-based targeting an increasingly feasible policy option, and the large number of aid programs that use mobile money as a distribution channel \citep{gentilini_social_2020} are well-placed for a shift to phone-based targeting. \color{black} Given the policy relevance of these results, we conclude by discussing important ethical and logistical considerations that may influence how CDR methods are used to support targeting efforts in practice.



% Research to date on wealth prediction from digital trace data has focused on mobile phone metadata as cell phones have become increasingly ubiquitous worldwide, projected to reach a global penetration rate of 70\% in 2025 \citep{gsma}.
%blumenstock2015,jean_combining_2016,ermon2019}.


 % While the idea that poverty is multidimensional is now well-established, how to apply these ideas to the assessment of targeting accuracy remains a challenge \citep{Alkire2015,Sen2010}. In this paper, we consider the hybrid approach selected by the government as the benchmark for capturing multidimensional poverty on which alternative targeting methods are compared against.  


% Given the success of wealth prediction from mobile phone data and the need for cheaper and more accurate targeting mechanisms in the LMICs, exploring poverty targeting based on CDR methods presents a natural extension of the existing literature. Here we build on the evidence on poverty targeting and wealth prediction from digital trace data to evaluate whether CDR data can be used in practice to target the very poor for anti-poverty programs. By matching CDR to household survey data from 535 households in 80 of the poorest villages in the Balkh province of Afghanistan, we assess whether CDR-based methods can replicate household-level targeting using a hybrid method from a recent program intended for ultra-poor households. We find that CDR-based targeting is as accurate as targeting based on assets or consumption for the subset of households that own a mobile phone in this sample, and that targeting based on a combination of assets, consumption, and CDR data is more accurate than targeting based on any one method assessed. We also analyze options for targeting the non-phone-owning ultra-poor household under CDR-based targeting regimes, noting in particular that allocating benefits to all non-phone-owning households does not compromise the accuracy of CDR-based targeting.%
%\footnote{JB add reference to \citet{aiken_machine_2021}.}
%We conclude by discussing the important ethical and logistical considerations that may influence how CDR methods are used to support targeting efforts in practice.



==> Targeting Paper_COPY2/intro_new.tex <==
% TODO

% Defining who is eligible for specific aid programs---targeting---has far-reaching economic and social implications. However, targeting can be costly, and often introduces significant errors of inclusion and exclusion \citep{alatas2012, alatas2016, brown2018, coady2004}. Finding cost-effective approaches to minimize targeting errors has become increasingly important within the global context of rapidly expanded social protection programs and increasing government debt. The visibility and importance of aid and aid targeting has increased dramatically in the past year: In 2020, global extreme poverty increased for the first time in two decades - driven by the COVID-19 pandemic, and exacerbated by the effects of conflict and climate change \citep{WorldBank_2020}. Most countries temporarily expanded their social protection programs in response to the pandemic, with more than 1.1 billion new recipients receiving government-led social assistance payments \citep{Gentilini2020}. 

% In high-income countries, targeting frequently relies on administrative data such as tax records or comprehensive social registries of poverty using metrics such as income or consumption. Low- and middle-income countries (LMICs), characterized by high levels of informality and a dearth of verifiable income data, typically follow alternative strategies that rely on primary data collection. However, feasibility of primary data collection and the reliability of these data are likely to introduce significant errors in the targeting process \citep{Deaton2016,jerven, wb_forthcoming}. These issues are exacerbated in fragile and conflict-affected countries, where two thirds of the world's poor are expected to reside by 2030 \citep{corral2020}. 


Recent studies have shown that non-traditional ``digital trace'' data---behavioral indicators recorded in everyday interactions with technology---are predictive of wealth in LMIC contexts \citep[e.g.][]{blumenstock2015, ermon2019}. There is optimism in the machine learning and development communities that these data could provide a quick and low-cost alternative or complement to standard field-based targeting methods, helping overcome logistical constraints to data collection, and increasing the cost-effectiveness of targeting  \citep[e.g.][]{blumenstock2016, dearteaga2018}.


In high-income countries, poverty targeting frequently relies on means-based testing, restricting program benefits to those below a certain income threshold based on administrative data such as tax records. In LMICs, means tests are often impractical due to high levels of informality. Traditional approaches in these countries rely on geographic targeting or proxy measures of economic well-being such as proxy-means testing (PMT), community-based targeting or a combination of these methods. PMTs use data on assets and demographic characteristics to create a proxy for consumption or income, while community-based methods allow community members and leaders to participate in the identification of eligible aid recipients. These approaches are imperfect, and inevitably lead to significant targeting errors; however, \cite{hannaolken} provide empirical evidence that narrowly-targeted programs can be significantly more cost-effective than widely-targeted programs or universal allocation, even when targeting is based on imperfect poverty proxies. 


Motivated by the importance of targeting for efficient allocation of development aid, a significant body of research has explored ways to improve targeting accuracy. 
A meta-analysis including 8 PMTs and 14 community-based targeting strategies finds that a similar level of resources went to the poorest 40\% in both community-based and PMT-based targeting methods \citep{coady2004}. Similarly, recent experimental evidence finds that differences in targeting errors across PMT, community-based and hybrid methods in Indonesia, India, Mali, Peru, Honduras and Niger, are often small relative to the base level of targeting errors using different benchmarks of well-being \citep{alatas2012,banerjee2007,Fortinetal2016,karlan2013,Premandetal2020}.\footnote{\citep{coady2004} find that targeting turned out to be regressive in a quarter of programs reviewed. This highlights the inherent challenges with measurement. Consumption and poverty estimates are based on surveys with quality issues, and ``in some cases, the problems are severe enough to threaten even the most basic understanding of growth, poverty and inequality" \citep{Deaton2016}.}
  
While \textit{per capita} consumption is often used as a benchmark to estimate poverty and measure targeting errors, the evidence comparing PMT and community-based approaches suggests that communities may apply a broader concept of poverty---for instance, including factors that predict earnings capacity. Community-based methods also typically yield higher rates of community satisfaction levels than PMT methods, when elite capture is absent. \citep{alatas2012,banerjee2007,Fortinetal2016,karlan2013,Premandetal2020}.\footnote{Contrary to this evidence, a study in Cameroon finds that community-based targeting methods performed consistently worse compared to PMT selection when assessed against consumption. However, the authors explained, that these are in part driven by communities including human and physical capital asset holding in the selection criteria---consistent with a multidimensional concept of poverty---and also due to implementation issues, reflected in errors of exclusion and inclusion above 40\% for PMT \citep{Stoeffler2016}}. While the idea that poverty is multidimensional is now well-established, how to apply these ideas to the assessment of targeting accuracy remains a challenge \citep{Alkire2015,Sen2010}. In this paper, we consider the hybrid approach selected by the government as the benchmark for capturing multidimensional poverty on which alternative targeting methods are compared against.  

Regardless of their accuracy (or inaccuracy), the current methods available for poverty targeting in LMICs are time- and resource-intensive, and  may be infeasible in fragile or conflict-affected areas or in contexts when mobility and social interaction is limited, such as during the current pandemic. We turn, therefore, to the literature on using passively collected digital trace data to estimate wealth, and later evaluate whether methods based on these data are useful for identifying the poor and the very poor. 



\subsubsection{Wealth Estimation from Mobile Phone Metadata}

Research to date on wealth prediction from digital trace data has focused on mobile phone metadata as cell phones have become increasingly ubiquitous worldwide, projected to reach a global penetration rate of 70\% in 2025 \citep{gsma}. Recent work has shown that machine learning methods leveraging CDR can produce useful estimates of wealth and well-being at a fine spatial granularity. This body of work focuses largely on poverty, typically quantified by an asset-based wealth index \citep[e.g.][]{blumenstock2015, hernandez}, but related papers explore a wider set of well-being measures, including literacy \citep{schmid}, food security \citep{decuyper1}, and infrastructure \citep{blumenstock2017}.

While most of this work addresses spatially granular poverty mapping, to our knowledge two papers to date cover the individual-level wealth prediction task that is more relevant to poverty targeting. \cite{blumenstock2015} show that CDR data are predictive of an individual-level asset-based wealth index in Rwanda. More specifically, the study matches ground-truth survey data to call detail records covering two years of mobile phone activity for 856 geographically stratified individuals, extracts a suite of thousands of behavioral indicators from the CDR covering different aspects of mobile phone use, and applies a supervised learning algorithm to generate wealth predictions from behavioral indicators. Model accuracy is evaluated with cross-validation to ensure that the wealth prediction model generalizes out-of-sample (cross-validated $r$ = 0.68). \cite{blumenstock2018} performs the same experiment for 1,234 male heads of households in the Kabul and Parwan districts of Afghanistan, yielding similar predictive accuracy.

\subsection{Our Contribution}

Given the success of wealth prediction from mobile phone data and the need for cheaper and more accurate targeting mechanisms in the LMICs, exploring poverty targeting based on CDR methods presents a natural extension of the existing literature. Here we build on the evidence on poverty targeting and wealth prediction from digital trace data to evaluate whether CDR data can be used in practice to target the very poor for anti-poverty programs. By matching CDR to household survey data from 535 households in 80 of the poorest villages in the Balkh province of Afghanistan, we assess whether CDR-based methods can replicate household-level targeting using a hybrid method from a recent program intended for ultra-poor households. We find that CDR-based targeting is as accurate as targeting based on assets or consumption for the subset of households that own a mobile phone in this sample, and that targeting based on a combination of assets, consumption, and CDR data is more accurate than targeting based on any one method assessed. We also analyze options for targeting the non-phone-owning ultra-poor household under CDR-based targeting regimes, noting in particular that allocating benefits to all non-phone-owning households does not compromise the accuracy of CDR-based targeting.%
\footnote{JB add reference to \citet{aiken_machine_2021}.}
We conclude by discussing the important ethical and logistical considerations that may influence how CDR methods are used to support targeting efforts in practice.



==> Targeting Paper_COPY2/methods.tex <==
%Our main analysis evaluates the extent to which machine learning and mobile phone data can  differentiate between ultra-poor and non-ultra-poor households in rural Afghanistan. This section describes the study population, the key datasets, and methods used to perform the evaluation.

\subsection{Household Survey Data}
\label{section:groundtruth}
Our empirical analysis relies on survey data collected as part of the Targeting the Ultra-Poor (TUP) program implemented by the government of Afghanistan with support from the World Bank. The TUP program was a ``big push," providing multi-faceted benefits to 7,500 ultra-poor households in six provinces of Afghanistan between 2015 and 2018 \citep{bedoya2019}. Our analysis uses data from the baseline and targeting surveys for an impact evaluation of the TUP program conducted in 80 of the poorest villages of Balkh province between November 2015 and April 2016 (N=2,582).\footnote{Our analysis restricts to 2,814 households for whom consumption and asset data are non-missing.}
%These data include interviews with nearly all of the 1,173 ultra-poor households in surveyed villages, and a random sample of 1,679 non-ultra-poor households.

\paragraph{Ultra-Poor Designation} Eligibility for the TUP program was determined based on based on geographic criteria,\footnote{The poorest villages were identified by the availability of veterinary services, financial institutions, and social services, and being relatively accessible \citep{bedoya2019}.}
followed by a two-step process including a community wealth ranking (CWR) and a follow-up in-person survey. CWRs were conducted separately in each village, coordinated by a local NGO and village leaders, in collaboration with the government team. %CWRs divided households into four categories: well-off (6\%), better-off (18\%), poor (33\%), and extreme-poor (43\%). 
The CWR was followed by an in-person survey to determine whether nominated households met a set of qualifying criteria, coordinated by the NGO and government representatives, and based on a measure of multiple deprivation. 

For a household to be designated as \textit{ultra-poor}, and therefore eligible for program benefits, it had to be considered extreme-poor in the CWR (43\% of households), and also meet at least three of six criteria:%
%\footnote{While these were the official criteria used to guide selection, they were not always strictly enforced --- see \citet{bedoya2019}.} 
\begin{enumerate}
\item Financially dependent on women's domestic work or begging
\item Owns less than 800 square meters of land or living in a cave
\item Primary woman under 50 years old
\item No adult men income earners
\item School-age children working for pay
\item No productive assets
\end{enumerate}

Ultimately, 11\% of the households classified as extreme-poor in the community wealth ranking step --- 6\% of the total population in the study villages --- were classified as ultra-poor and eligible for TUP benefits. Of the 2,852 households surveyed for the TUP project, 1,173 (41\%) were designated as ultra-poor, and 1,679 (59\%) were non-ultra-poor.%
\footnote{Surveys were conducted following the CWR and eligibility verification. The response rate for ultra-poor households was 96\%. Approximately 20 households in each of the study villages were randomly drawn (excluding TUP-eligible households), to provide a representative benchmark for the TUP sample.} 

\paragraph{Consumption} The consumption module of the TUP survey contains information on food consumption for the week prior to the interview and non-food expenditures for the year prior to the interview. These are used to construct monthly \textit{per capita} consumption values, as detailed in \cite{bedoya2019}. Based on these data, we measure the logarithm of \textit{per capita} monthly consumption, using the same approach that the Afghan government used to determine the national poverty line.  %Figure \ref{expenddist} shows the distribution of per-capita consumption and log-transformed per-capita consumption in our 537-household sample. The Afghanistan national poverty line for 2016-2017 is AFN 2,064 (equivalent to USD 112 PPP) per person per month. In our dataset, determination of poverty line status is based on a poverty-line consistent measure of consumption, which includes food consumption, consumer durables, housing costs, and a subset of the non-food costs included in the standard consumption calculation. 53\% of our 537-household sample is below the poverty line and 47\% is above the poverty line.

\paragraph{Asset Index} We construct an asset-based wealth index to assess the relative socioeconomic status of surveyed households, calculated as the first principal component of variation in household asset ownership for sixteen items in Table \ref{appendix:firstcomponent}. The principal component analysis is calculated across the 2,814 households with complete asset data, after standardizing each asset variable to zero mean and unit variance. This wealth index explains 25.3\% of the variation in asset ownership. Figure \ref{appendix:assetindex} shows the distribution of the underlying asset index components and Table \ref{appendix:firstcomponent} shows the direction of the first principal component. %We winsorize the wealth index with a 99\% limit. %Figure \ref{distributions} shows the distribution of each of the individual components and of the composite wealth index for the 537 households in our sample. 

%\begin{figure}[H]
%\centering 
%\includegraphics[width=1\columnwidth]{fig1part1.png}
%\includegraphics[width=1\columnwidth]{fig1part2.png}
%\caption{Distribution of asset-based wealth index and individual asset ownership across 537 households.} 
%\label{distributions} 
%\end{figure}



%\begin{figure}[H]
%\centering 
%\includegraphics[width=1\columnwidth]{dist_expend.png}
%\caption{Distribution of consumption across 537 households pre- and post- log transformation.} 
%\label{expenddist} 
%\end{figure}

%\paragraph{Poverty Line} The Afghanistan national poverty line for 2016-2017 is AFN 2,064 (equivalent to USD 112 PPP) per person per month. In our dataset, determination of poverty line status is based on a poverty-line consistent measure of consumption, which includes food consumption, consumer durables, housing costs, and a subset of the non-food costs included in the standard consumption calculation. 53\% of our 537-household sample is below the poverty line and 47\% is above the poverty line.

\paragraph{Other Variables} The TUP surveys collected several other covariates that we use in subsequent analysis. These include a food security index (composed of variables relating to the skipping and downsizing of meals, separately for adults and children), a financial inclusion index (composed of access to banking and credit, knowledge of banking and credit, and savings), and a psychological well-being index for the primary woman (standardized weighted scores on the Center for Epidemiological Studies Depression scale, the World Values Survey happiness and satisfaction questions, and Cohen's Stress Scale) -- see \citet{bedoya2019}. The survey also collected data from each household on mobile phone ownership. Nearly all (99\%) households with a cell phone provided their phone numbers and consented to the use of their call detail records for this study.   

\paragraph{Sample Representativity} 
\label{section:selectionintosample}
Portions of our analysis are restricted to the 535 households from the TUP survey with phone numbers that match to our CDR (see Section \ref{section:cdr}). Table \ref{selectionintosample} and~\ref{appendix:kdeoutcomes} compare characteristics of these households to the full survey population. 
There are some systematic differences: the 535-household sample is wealthier, which is consistent with households in the subsample being required to own at least one phone.  For instance, while 88\% of non-ultra-poor households in the TUP survey own at least one phone, only 72\% of ultra-poor households own at least one phone. %In contrast, only 43.3\% of individuals in the ALCS survey report owning a mobile phone (though at least part of this difference can be attributed to the inconsistency of household vs. individual-level data).

\paragraph{Summary Statistics} 
As shown in Table \ref{selectionintosample} and Figure \ref{appendix:correlations}, the  three measures of well-being in our dataset are only weakly correlated with one another: for example, the correlation between the asset index and consumption is 0.37 in the full survey and 0.34 in the matched subsample. Likewise, while the ultra-poor population makes up 27\% of the overall sub-sample, less than half of the ultra-poor fall into the bottom 27\% of the sample by wealth index or consumption.

\paragraph{Sample Weights} Since the TUP survey oversampled the ultra-poor (by a factor of roughly 12), portions of our analysis use sample weights to adjust for population representativity. When sample weights are applied, it is explicitly noted; if not mentioned, no weights are applied. %The sample weights are derived from the population of the village, and the household's ultra-poor designation.%
%\footnote{A census listing was conducted in each village to facilitate the CWR exercise. In some cases, large villages were split into smaller units and weights are based on the sub-village.} 
After sample weights are applied, the ultra-poor make up 5.98\% of the overall population, and 4.63\% of our matched subsample. 
%\paragraph{Comparison of Outcome Measures} %While all the wealth measures in our dataset are correlated with one another, none are completely overlapping. Even the poverty line indicator, which is a consumption-based measure, differs slightly from the consumption outcome since it is based on a somewhat different set of costs. 

%Table \ref{corrmatrix} displays the correlations among wealth measures, while %Figure \ref{measurecomparison} visualizes the overlap among the different outcome measures. 


%\begin{table}[H]
%\centering
%\footnotesize
%\input{tables/wealthmeasure_correlations_new}
%\caption{Correlations between outcome measures, separately for just the households matched to CDR (Panel A) and all households from the TUP baseline survey with all three ground truth poverty measures recorded (Panel B).} 
%\label{corrmatrix} 
%\end{table}

%\begin{figure}[H]
%\centering 
%\includegraphics[width=1\columnwidth]{wealthscorescomparison.png}
%\caption{Comparison of wealth measures: wealth score vs. consumption by ultra-poor and poverty-line status.} 
%\label{measurecomparison} 
%\end{figure}

\subsection{Mobile Phone Metadata} 
\label{section:cdr}

In a follow-up survey conducted in 2018, we requested informed consent from survey respondents to obtain their mobile phone CDR and match them to the survey data collected through the TUP project. CDR contain detailed information on:

\begin{itemize}
    \item \textbf{Calls: } Phone numbers for the caller and receiver, time and duration of the call, and cell tower through which the call was placed
    \item \textbf{Text messages: } Phone numbers for the caller and recipient, time of the message
    \item \textbf{Recharges: } Time and amount of the recharge
\end{itemize}

For participants who consented, we match baseline survey data (collected November 2015 - April 2016) to CDR covering that same period, obtained from one of Afghanistan's main mobile phone operators. For households with multiple phones and a designated household head (N=65), we match to CDR for the phone belonging to the household head. For households where the household head does not have a phone and someone else does (N=17), we match to CDR for one of the households' phones selected at random. In total, for the 535 households in our sample, 629,543 transactions took place in the months of November 2015 to April 2016, broken down into 310,883 calls, 305,756 text messages, and 12,904 recharges.%\footnote{While our main analysis is done at the household level, we later explore an alternative approach that matches survey data reported by the household head to all phone numbers associated with the household.}

From these CDR, we compute a set of 797 behavioral indicators that capture aggregate aspects of each individual's mobile phone use \citep{bandicoot}. This set includes indicators relating to an individual's communications (for example, average call duration and percent initiated conversations), their network of contacts (for example, the entropy of their contacts and the balance of interactions per contact), their spatial patterns based on cell tower locations (for example, the number of unique antennas visited and the radius of gyration), and their recharge patterns (including the average amount recharged and the time between recharges). %Each indicator is computed separately for weekdays, weekends, daytime, and nighttime activity. %
The distributions of a sample of these indicators are shown in Figure~\ref{appendix:feature_kdes}.

\subsection{Machine Learning Predictions} 

\paragraph{CDR-based Method} Extending the approach described in \citet{blumenstock2015}, we test the extent to which ultra-poor status can be predicted from CDR. This analysis uses the 535 TUP households who match to CDR to train a supervised machine learning algorithm to predict ultra-poverty status from the mobile phone features. The intuition --- also highlighted in Figure~\ref{appendix:feature_kdes} --- is that ultra-poor individuals use their phones very differently than non-ultra-poor individuals, and machine learning algorithms can use those differences to predict ultra-poor status.

Our main analysis uses a gradient boosting model, which generally out-performs several other common machine learning algorithms for this task (see Table~\ref{appendix:mldetails}). The feature importances for the trained model are shown in Table~\ref{appendix:importances}. To limit the potential for overfitting, probabilistic predictions are generated via 10-fold cross-validation, with folds stratified to preserve class balance.\footnote{While cross validation is a standard evaluation strategy in the machine learning literature, for robustness we present results using a basic single train-test split in Table \ref{onesplit}.} %We tune hyperparameters using five-fold cross-validation for each  fold separately.%
Additional details on the machine learning methods are provided in Appendix \ref{appendix:ml}.

%, our main analysis highlights the results of the gradient boosting model, which generally performs better than alternative methods. We also extract feature importances for our preferred model, which are displayed in Table \ref{appendix:importances} and Figure \ref{appendix:feature_kdes}.



\paragraph{Combined Methods} We also evaluate several approaches that use data from multiple sources to predict ultra-poor status. Our main \textit{combined method} trains a logistic regression to classify the ultra-poor and non-ultra-poor households using the predicted ultra-poor probability from the CDR-based method (i.e., the output of the gradient boosting algorithm described above), as well as asset and consumption data collected in the TUP survey. For comparison, we similarly evaluate the performance of methods that combine only two of the available data sources (i.e., assets plus consumption, assets plus CDR, and consumption plus CDR). Predictions for each of the combined methods are pooled over 10-fold cross-validation.

\subsection{Targeting Accuracy Evaluation}
\label{section:evaluation}

\paragraph{Evaluation on Matched Subsample} Our main analysis focuses on the 535 households for which we observe both CDR and survey data, and evaluates whether machine learning methods leveraging CDR data can accurately identify households designated as ultra-poor by the TUP program (using the two-step hybrid approach described in Section~\ref{section:groundtruth}). We compare the performance of the CDR-based method to the performance of methods based on the wealth index, consumption data, and combinations of these data sources.%
\footnote{The CDR-based method uses supervised learning to model the ultra-poverty outcome, whereas the asset- and consumption-based approaches do not. To assess the importance of this difference, we experiment with applying machine learning methods to the asset and consumption data to model the ultra-poverty outcome. In results shown in Table~\ref{appendix:assetbasedpred}, we find that a machine-learned asset predictor provides slight improvements on the standard asset-based wealth index and consumption measures. We continue to use the standard asset and consumption measures as benchmarks in the remainder of the paper, however, as they are the targeting methods most frequently used in practice.}
Each targeting method is evaluated based on classification accuracy, errors of exclusion (ultra-poor households misclassified as non-ultra-poor) and errors of inclusion (non-ultra-poor households misclassified as ultra-poor). 
We focus on the ultra-poor designation as the `ground truth' status of the household, against which other methods are evaluated, since it is the most carefully vetted measure of well-being for this population, and the proxy that the government used to target TUP benefits.

To evaluate the performance of the CDR-based and combined methods, we pool out-of-sample predictions across the ten cross-validation folds, so that every household in our dataset is associated with a CDR-based predicted probability of ultra-poor status that is produced out-of-sample.\footnote{In Table~\ref{onesplit}, we show that results are unchanged when we use a single train-test split, instead of 10-fold cross-validation.} To account for class imbalance, we evaluate model accuracy using a ``quota method", by selecting a cut-off threshold for ultra-poor qualification such that each method identifies the proportion of ultra-poor households in our subsample; this cut-off also balances inclusion and exclusion errors. This quota-based approach reflects a scenario in which a program has a fixed budget constraint; it is  also frequently used in the targeting literature \citep{alatas2012, schnitzer2021targeting}. In our 535-household matched dataset this threshold is 27\%; in other samples (see following subsection), the percentage is different. We evaluate each method for precision (positive predictive value) and recall (sensitivity). To capture the trade-off between inclusion and exclusion errors for varying values of this threshold, we also construct receiver operating characteristic (ROC) curves for each method and consider the area under the curve (AUC) as a measure of targeting quality. For each evaluation metric (precision, recall, and AUC), we bootstrap 1,000 samples from the original dataset to calculate the standard deviation of the mean of the accuracy metric. Each bootstrapped sample is of the same size as the original dataset, drawn with replacement.

%\paragraph{Reweighting for Population Representivity and Non-Phone Owning Households}
\paragraph{Accounting for Households Without Phones} 
Our main results assess the performance of different targeting methods on the sample of 535 households for whom we have both survey data and mobile phone data. 
We also present results that show how performance is affected when the analysis includes TUP households for whom we do not have mobile phone data (typically because they do not have a phone or because they use a different phone network than the one who provided CDR). We provide analysis that targets such households (1) before households with CDR, or (2) after households with CDR (see  Section~\ref{sec:nophones}). These results are evaluated on three different samples:

\begin{enumerate}
    \item \textit{Matched Sample:} The 535 households for whom could match survey responses to CDR.
    
%    \item 535 households with matched survey and CDR data available, with sample weights applied.
    \item \textit{Balanced Sample:} This sample includes the 535 matched households as well as the 472 households in the TUP survey who report not owning any phone. It excludes households that own a phone on a different phone network than the one who provided CDR. The motivation for this sample is to provide an indication of targeting performance in a regime in which CDR can be used to target all phone-owning households. In addition to applying sample weights from the survey, households that do not own a phone are downweighted so that the balance of phone owners to non-phone-owners (with sample weights applied) is the same as in the baseline survey as a whole (with sample weights applied, 84\% phone owners).

    \item \textit{Full Sample:} All 2,814 households in the TUP baseline survey for which asset and consumption data are available, with sample weights applied.

\end{enumerate}

Note that the quota used to evaluate targeting changes for each sample, based on the number of households that are ultra-poor in the sample. For the matched sample, the targeting quota is 27.29\%; for the balanced sample and full sample the quotas are 5.47\% and 6.02\%, respectively. 


%The 535-household matched sample is biased in important ways in comparison to the TUP survey. To evaluate the accuracy of CDR-based targeting methods with incomplete mobile phone penetration, we also present scenarios augmenting our sample with data from non-phone-owning households from the TUP survey. Specifically, we perform targeting simulations with the following four samples:


==> Targeting Paper_COPY2/results.tex <==
%\subsection{Identifying the Ultra-Poor Among Households Matched to CDR}

\subsection{Performance of Targeting Methods}
Our first set of results evaluate the extent to which different targeting methods can correctly identify ultra-poor households. This analysis compares the performance of CDR-based targeting methods to asset-based and consumption-based targeting, using the sample of 535 households for which survey data and CDR data are both available. 

%27\% of these households are ultra-poor. Due to class imbalance, we evaluate errors of inclusion and exclusion by choosing a decision threshold where the correct number of households are identified as ultra-poor --- this threshold also balances errors of inclusion and exclusion. 
An overview of these results is provided in Figure \ref{targeting}. Figure \ref{targeting}a shows the distribution of assets and consumption, as well as the distribution of predicted probabilities of being non-ultra-poor generated by the CDR-based and combined methods, separately for the ultra-poor and non-ultra-poor. The dashed vertical line indicates the threshold at which point 27\% of households are classified as ultra-poor; we use this quota because 27\% of households in this sample were designed as ultra-poor by TUP. Figure \ref{targeting}b provides confusion matrices that compare the true status (rows) against the classification made by each method (columns). These confusion matrices are also used to calculate the measures of precision and recall reported in Table \ref{resultstable} Panel A.

We find that the CDR-based method (precision and recall of 42\%) is close in accuracy to methods relying on assets (precision and recall of 49\%) or consumption (precision and recall of 45\%). To evaluate the trade-off between inclusion errors and exclusion errors resulting from selecting alternative cut-off thresholds, Figure \ref{targeting}c shows the ROC curve associated with each classification method, and the associated Area Under the Curve (AUC). AUC scores  are comparable among methods, with assets (AUC=0.73) slightly superior to consumption (AUC=0.71) and the CDR-based method (AUC=0.68).% After applying sample weights, these scores transform slightly to AUC = 0.73, 0.70, and 0.66 for assets, consumption, and CDR respectively, as detailed in Table \ref{resultstable} Panel B.

\subsection{Comparison of Errors Across Methods}
To better understand where the targeting methods are making mistakes, Panel A of Table \ref{tp_vs_fn} indicates how the ultra-poor misclassified as non-ultra-poor (false negatives) compare to the correctly classified ultra-poor (true positives). Panel B shows how the non-ultra-poor misclassified as ultra-poor (false positives) compare to the correctly classified non-ultra-poor (true negatives). 

 Across methods, false negatives score higher on food security, financial inclusion, and psychological well-being than true positives -- that is, all three targeting methods misclassify ultra-poor households as non-ultra-poor when those ultra-poor households are better-off, according to other observable characteristics not used in the targeting.  Likewise, false positives (non-ultra-poor misclassified as ultra-poor) tend to score lower than true negatives across these same measures. The CDR-based method in particular tends to prioritize households that score low on these alternative measures of well-being.

To test for systematic misclassification of certain types of households, Table \ref{mistakesoverlapexclusion} displays the overlap in errors of exclusion and inclusion between methods. Our results suggest that the three classifiers misidentify the same households at a rate only slightly above random.%
\footnote{The rates of overlap should be interpreted relative to the expected overlap in errors for random classifiers. Based on our selection of thresholds such that 27\% of the sample is identified as ultra-poor, our three classifiers misidentify 15-27\% of the non-ultra-poor and 51-65\% of the ultra-poor. If these classifiers were random, we would expect approximately 20\% overlap in inclusion errors and 55\% overlap in exclusion errors.}

\subsection{Combining Targeting Methods}
Since the different targeting methods identify different populations as ultra-poor, there may be complementarities between asset, consumption, and CDR data. As shown in Panel A of Table \ref{resultstable}, we find that a \textit{combined method},  which takes as input the wealth index, total consumption, and the output of the CDR-based method, performs better (AUC = 0.78) than methods using any one data source (AUC = 0.68 - 0.73). As shown in Table~\ref{appendix:combined}, the full method also outperforms methods based on any two data sources (AUC = 0.75 - 0.76). The method that combines CDR and asset data (AUC = 0.76) may, however, be more practical than the combined method, since consumption data is difficult to collect for large populations.

\subsection{Targeting Households Without Phones}
\label{sec:nophones}
An important limitation of CDR-based targeting is that households without phones do not generate CDR. %Section~\ref{sec:discussion} discusses broader implications for program design; for now, we present results that show how predictive performance is impacted by the inclusion of these households in the analysis.
Here, we show how targeting performance is impacted when households without phones are included in the analysis. This analysis uses two additional samples of TUP households to evaluate targeting performance: (i) the \textit{balanced sample}, which adds all of the 472 households without phones to the sample of 535 for whom we have matched CDR; the balanced sample is intended to illustrate the performance of CDR-based targeting if CDR were available from all operators in Afghanistan --- though it relies on the assumption that phone-owners observed on our mobile network are representative of all phone owners in Afghanistan (an assumption that is not fully satisfied, as shown in Table \ref{selectionintosample}); and (ii) the \textit{full sample}, which includes all 2,814 households surveyed in the TUP baseline; this sample includes an additional 1,807 households who report owning a phone, but whose number does not match to any number in the CDR provided to us by the single mobile operator.%
\footnote{These 1,807 households include households that report owning a phone on a different network (this network is estimated to have around 30\% market share in Afghanistan), as well as phones on our network that were not active during the six-month period of CDR that we analyze.}

Results in Panels B and C of Table~\ref{resultstable} show the performance of each targeting approach on the balanced and full sample, respectively. Note that as described in Section \ref{section:evaluation}, different targeting quotas are applied for each panel based on the proportion of each sample that is ultra-poor. In the CDR-based and combined approaches, we report performance when the households without CDR are targeted first (i.e. households without CDR are targeted in a random order and then the households predicted to be poorest are targeted until the quota is reached) as well as when households without CDR are targeted last (i.e., after the 535 households with phones are targeted, households without phones are included in a random order until the quota is reached).

Unsurprisingly, these results suggest that CDR-based targeting is not effective when a large portion of the target population does not own a phone (e.g. Panel C of Table~\ref{resultstable}, where only 16\% of the sample has matching CDR). However, when we simulate more realistic levels of phone ownership in Panel B (84\% of the households, based on our survey data), CDR-based targeting is once again comparable to asset- or expenditure-based targeting, particularly when households without phones are targeted first (AUC = 0.72, 0.70, 0.68 for assets, consumption, and CDR, respectively). On the other hand, if households without phones are targeted last (for example, if program administrators base targeting wholly on CDR and provide no benefits to any household without a phone), the CDR-based method only improves marginally on random targeting.


\subsection{Additional tests and simulations} 

Our main analysis considers the household head to be the unit of analysis. As described in Section~\ref{section:cdr}, this analysis is based on matching survey-based indices to phone data from the household head, which is consistent with the design of the TUP program and the TUP survey sample frame. An alternative approach matches survey data reported by the household head to all phone numbers associated with the household. As shown in Table~\ref{appendix:individual}, the predictive accuracy of these models is slightly attenuated relative to the benchmark results (Table~\ref{appendix:mldetails}).

We also explore the extent to which CDR can be used to predict other measures of socioeconomic status. Our main analysis focuses on the household's ultra-poor designation as the ground truth measure of poverty, since this label was both carefully curated and the actual criterion used to determine TUP eligibility. In Table~\ref{appendix:mlresults}, we report the accuracy with which CDR (obtained from the household head, who is typically male) can predict consumption and asset-based wealth (elicited from the primary woman of each household).%
\footnote{Due to the design of the TUP survey, which interviewed women in the household, we cannot avoid this mismatch between the survey respondent and the phone owner.}
In general, these machine learning models trained to directly predict consumption or asset-based wealth do not perform well. This result contrasts with prior work documenting the predictive ability of CDR for measuring asset-based wealth \citep[e.g.][]{blumenstock2015}. We suspect a key difference in our setting -- aside from the fact that we are matching CDR to socioeconomic status at the \textit{household} rather than the \textit{individual} level -- is the homogeneity of the beneficiary population: whereas \citet{blumenstock2015} uses machine learning to predict the wealth of a nationally-representative sample of Rwandan phone owners, our sample consists of 535 individuals from the poorest villages of a single province in Afghanistan, where even the relatively wealthy households are quite poor. 

%\subsection{Targeting Costs}

%Our final set of results compare the approximate costs of implementing each of the targeting methods. We compare variable costs per household screened for CBT and PMT-based targeting taken from the literature (Table \ref{appendix:costliterature}) to simulated costs of phone-based targeting in Table \ref{appendix:costs}. While CBT and PMT-based targeting for the entire TUP program, which covered six provinces, would cost an estimated \$140,153 and \$254,824 respectively (2.23\% and 4.06\% of the budget spent on program benefits), the variable costs for phone-based targeting could be as low as zero. However, if informed consent to analyze phone data were collected from every household prior to implementing phone-based targeting, costs would rise: in person informed consent could be almost as expensive to collect as a PMT or CBT exercise; collected informed consent over the phone via an SMS or call could be substantially cheaper.

%Another likely factor limiting the extent to which CDR can predict consumption in that the TUP interviews were conducted with the primary woman of each household. However, for most households, CDR was obtained from the household head, who was typically male. Thus, the results in Table~\ref{appendix:mlresults} 
%so that frequently in these experiments survey responses are being matched to CDR of individuals not directly surveyed (in contrast to our main experiment of predicting ultra-poor status, where ultra-poor status was determined at the household level in a community wealth ranking). 

%Our main analysis studies the degree to which asset-based, consumption-based, and CDR-based methods can identify ultra-poor households. In other contexts, however, it may be more valuable to understand how CDR compares to other methods when it comes to targeting households based on other metrics of poverty, such as consumption or wealth. Table \ref{appendix:mlresults} documents the extent to which CDR can predict a set of poverty measures, including consumption, the asset index, below poverty line or extreme poverty line (based on consumption), and the wealth ranking from the CWR group.  We find that CDR has little predictive power for most other poverty measures.

% Consumption is of particular interest in many targeting applications. Table \ref{appendix:consumption} evaluates the extent to which three targeting methods (asset index, ultra-poverty as defined in the hybrid targeting method used for the TUP program, and CDR-predicted consumption) can identify the 27\% consumption-poorest households in the 535-household matched sample. We find that the CDR-based method is no better than random for identifying the poorest households by consumption, while assets and ultra-poverty are both better than random targeting. 


%Three simple methods for addressing this issue are 1) targeting households without a phone first, 2) targeting households without a phone last, and 3) targeting households without a phone at random.  In this section, we simulate these three options using data from all 2,814 households from the TUP survey, rather than only the 535 households with matched CDR data analyzed earlier.

%Table \ref{resultstable} presents simulations of targeting methods with four subtly different samples: first, the 535 households with matched CDR without sample weights applied, as in the earlier analysis; second, the same households with sample weights applied; third, all 2,814 households in the TUP baseline survey, with sample weights applied, and fourth, the 1,007 households in the TUP survey that either own a phone matched to CDR or no phone at all, with phone-owning households upweighted so that the ratio of phone-owning to non-phone owning households is the same as in the full 2,814-household sample (84\% phone ownership). This fourth sample simulates what CDR-based targeting could look like in practice if CDR for all phone-owners were available, though it relies on the assumption that phone-owners observed on our mobile network are representative of all phone owners in Afghanistan (an assumption that is not fully satisfied, as shown in Table \ref{selectionintosample}). 


%Unsurprisingly, these results suggest that no CDR-based method is effective when only 18\% of the households owns a phone. However, when we simulate more realistic levels of phone ownership (84\% of the households, based on our survey data), we note that CDR-based targeting is once again comparable to asset- or expenditure-based targeting, particularly when households without phones are targeted first (AUC = 0.72, 0.70, 0.68 for assets, consumption, and CDR, respectively). On the other hand, if the CDR-based method is used and households without phones are targeted last (for example, if program administrators base targeting wholly on CDR and provide no benefits to any household without a phone), the CDR-based method only improves marginally on random targeting.

%\begin{table}[H]
%\centering
%\footnotesize
%\input{tables/weighting}
%\caption{Summary  of  accuracy  across  methods  using  different  sampling  strategies. The  sample  used  in  Panel  A is  all  households  with  a  phone  that  was  active  in  our mobile network  dataset  between  November  and  April  2016. This sample is biased due to 1) separate sampling processes for ultra-poor and non-ultra-poor households resulting in a higher percentage of ultra-poor households in the subsample than in the population, and 2) the requirement that all households in the subsample own a phone that appears in our CDR dataset. Panel B applies sample weights associated with each household in the matched subsample. Note that there are several types of households in the population which are are left out of this subsample: households that do not own a phone, households that own a phone that is not on our network, and households that have inactive phones.  Our data suggest that most households that are not included in the Panels A and B samples either own an inactive phone or own a phone that is not in our CDR dataset;  only  17.23\%  (weighted)  of  households  outside  of  the  Panel  B  sample  report  not  owning  a  phone. Panel C uses sample weights from all households in the baseline survey to evaluate targeting in the general population.  For CDR-based targeting methods, we consider the options of labelling all non-phone-owning households as ultra-poor and all non-phone-owning households as non-ultra-poor. Panel D uses observations only from matched households and non-phone-owning households, upweighting all households in the matched sample to estimate population-level accuracy if all phone-owners had matched CDR. The implicit assumption here is that phone-owners outside our matched sample are comparable to phone-owners within our sample.} 
%\label{weighting} 
%\end{table}

%\begin{figure}[H]
%\centering 
%\includegraphics[width=1\textwidth]{weighting.png}
%\caption{ROC curves for targeting methods under the same four simulations as in Table \ref{weighting}. Circles mark the targeting cut-off where as many households are targeted as are truly ultra-poor.} 
%\label{weighting_rocs} 
%\end{figure}

%\subsection{Comparison of Predictive Accuracy Across Wealth Measures}

%For comparison with past work on poverty estimation from CDR data, we also evaluate the ability of CDR-based methods to predict the asset-based wealth index, consumption, and an indicator for being above or below the poverty line in our sample. We begin with an in-sample analysis, comparing the relationship between behavioral features from CDR data and ground-truth survey-based measures of welfare across our 537-household sample. We then evaluate the accuracy of machine learning models leveraging CDR data for out-of-sample prediction of the four wealth measures based on CDR data.

%\paragraph {In-Sample Analysis} We perform a two-sided t-test to compare the mean of CDR features in the ultra-poor and non-ultra-poor samples, and find that 237 of the 623 CDR features have significantly different means in the two populations on a 0.05 level. With the same methodology, we find that 158 CDR features have significantly different means for populations above and below the poverty line. Kernel density estimates comparing the distributions of five of these behavioral features are included in Figure \ref{hists}.

%\begin{figure*}
%\centering 
%\includegraphics[width=1\textwidth]{hist.png}
%\caption{Comparing distributions of selected CDR features for ultra-poor vs. non-ultra-poor households (above) and above vs. below poverty line households (below). From left to right: number of active days of phone use, number of unique weeknight contacts (call or text), entropy of weekend contacts (call or text), number of unique antennas, and the churn rate (level of dissimilarity in spatial patterns between weeks, based on antenna locations).} 
%\label{hists} 
%\end{figure*}

%\begin{figure*}
%\centering 
%\includegraphics[width=1\textwidth]{corrs_537.png}
%\caption{Summary of correlations between CDR features and continuous wealth measures (wealth index above and consumption below). Left: Distribution of correlations between behavioral features extracted from CDR data and ground truth wealth measures. Right: Scatterplots showing the relationship between selected CDR features and ground truth wealth measures, with linear trend lines. From left to right: number of unique nighttime contacts (call or text), number of unique antennas, total calls, and total recharges.} 
%\label{eda} 
%\end{figure*}

%We also find that there is significant correlation between many of the behavioral CDR features and the continuous measures of wealth (wealth index and consumption); the distribution of correlations is shown in Figure \ref{eda}. However, we find that many of the CDR features most correlated with wealth are highly collinear. Moreover, many of the most useful CDR features are structurally related to one another: among the top 10 features most correlated with the wealth index, for example, nine are related to number of contacts. Surprisingly, in comparison to previous work \citep{steele2017}, we find weak correlations between recharge behavior and wealth (for example, the correlation between number of recharges and the wealth index is 0.09; there is no correlation between the average amount recharged and wealth index). Figure \ref{eda} shows the relationship between several intuitively interpretable CDR features and the wealth index and consumption in our sample.

%\paragraph{Out-of-Sample Prediction} While the differences in CDR feature distributions between ultra-poor and non-ultra-poor households and the correlations between CDR features and the wealth index suggest that there is promise for predicting wealth from behavioral CDR features in this dataset, it is possible that the in-sample model is overfit and has no out-of-sample predictive power. Out-of-sample prediction, in this case through cross-validation, is a better measure of the model's ability to predict an arbitrary individual's wealth from their mobile phone history. 

%As shown in Table \ref{allmeasures}, and in contrast to previous work, we find little predictive power for an asset-based wealth index (cross-validated $r$ = .03-.17), consumption (cross-validated $r$ = .01-.13), or the poverty line indicator (cross-validated AUC = .47-.58). As above, we find significantly more predictive power for the ultra-poor indicator (cross-validated AUC = .62-.70).

%\begin{table}[H]
%\centering
%\tiny
%\input{tables/accuracy_all}
%\caption{Accuracy for predicting four measures of wealth from CDR data. Continuous wealth measures (asset-based wealth index and consumption) are evaluated based on correlation ($r$) between true and predicted wealth, binary wealth measures (indicator for being below the poverty line and indicator for being ultra-poor) are evaluated for AUC score. Results presented are averages over 10-fold cross validation, with standard deviations in parentheses. The most accurate machine learning method for predicting each measure is bolded.} 
%\label{allmeasures} 
%\end{table}
%\vspace{2cm}

==> Targeting Paper_COPY2/supplementary_material.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% APPENDICES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Machine learning methods and hyperparameters}
\label{appendix:ml}

Although our paper is focused on identifying the ultra-poor with CDR, we experiment with predicting four measures of ground-truth welfare with CDR features: ultra-poor status (binary), below the national poverty line (binary), asset index (continuous), and log consumption (continuous). For the binary measures, we experiment with four classification models: logistic regression (unregularized), logistic regression with L1 penalty, a random forest, and a gradient boosting model. For the continuous measures, we experiment with four regression models: linear regression, LASSO regression, a random forest, and a gradient boosting model. The linear models and random forest are implemented in Python’s scikit-learn package. The gradient boosting model is implemented with Microsoft’s LightGBM. 

In each case, we produce predictions out-of-sample over 10-fold cross validation. We use nested cross-validation to tune the hyperparameters of each model over 5-fold cross-validation within each of the outer folds to avoid any information leakage between folds. We report both the mean score across the 10 folds as well as the overall score when data from all folds is pooled together. For the linear models and random forest, missing data is mean-imputed and each feature is scaled to zero mean and unit variance before fitting models (these transformations are done separately for each fold, with parameters fitted only on the training data for each fold). For the gradient boosting model missing values are left as-is and features are not scaled. We re-fit the model on the entire data, again tuning hyperparameters over 5-fold cross validation, to report selected hyperparameters and feature importances. We also report the top 5 features for each model, determined by the magnitude of the coefficient for the linear models, and by and by maximum impurity reductions for the tree-based models. 

Hyperparameters are selected from the following grids for each model:


\paragraph{Linear/Logistic Regression}
\begin{itemize}
    \item Drop columns with missingness over: \{50\%, 80\%, 100\%\}
    \item Drop columns with variance under: \{0, 0.01, 0.1\}
    \item Winsorization limit: \{0\%, 1\%, 5\%\}
\end{itemize}

\paragraph{LASSO Regression}
\begin{itemize}
    \item Drop columns with missingness over: \{50\%, 80\%, 100\%\}
    \item Drop columns with variance under: \{0, 0.01, 0.1\}
    \item Winsorization limit: \{0\%, 1\%, 5\%\}
    \item L1 penalty: \{0.00001, 0.0001, 0.001, 0.01, 0.1, 1, 10, 100\}
\end{itemize}

\paragraph{Random Forest}
\begin{itemize}
    \item Drop columns with missingness over: \{50\%, 80\%, 100\%\}
    \item Drop columns with variance under: \{0, 0.01, 0.1\}
    \item Winsorization limit: \{0\%, 1\%, 5\%\}
    \item Number of Trees: \{20, 50, 100\}
    \item Maximum Depth: \{1, 2, 4, 6, 8, 10, 12\}
\end{itemize}

\paragraph{Gradient Boosting Model}
\begin{itemize}
    \item Drop columns with missingness over: \{50\%, 80\%, 100\%\}
    \item Drop columns with variance under: \{0, 0.01, 0.1\}
    \item Winsorization limit: \{0\%, 1\%, 5\%\}
    \item Number of Trees: \{20, 50, 100\}
    \item Minimum data in leaf: \{5, 10\}
    \item Number of leaves: \{5, 10, 20\}
    \item Learning rate: \{0.05, 0.075\}
\end{itemize}

\pagebreak
\section{Abbreviations in Feature Names}
\label{appendix:abbreviations}

Figure \ref{appendix:feature_kdes} and Tables \ref{appendix:mlresults}, \ref{appendix:importances}, and \ref{appendix:individual} use a set of abbreviations in CDR feature names. This appendix lists the relevant abbreviations.

\begin{itemize}
    \item BOC: Balance of contacts
    \item CD: Call duration
    \item IPC: Interactions per contact
    \item IT: Interevent time
    \item NOI: Number of interactions
    \item PPD: Percent pareto durations (percentage of call contacts accounting for 80\% of call time)
    \item PPI: Percent pareto interactions (percentage of contacts accounting for 80\% of subscriber's interactions)
    \item RD: Response delay
    \item RR: Response rate
    \item WD: Weekday 
    \item WE: Weekend
\end{itemize}

\section{Cost and Speed Calculations}
\label{sec:appendix:costs}
In the discussion section we provide a cost and speed comparison between targeting methods, as some of the value-add of the phone-based targeting approach relies on how cheap and quick it is compared to asset, consumption- or CBT-based targeting approaches. Administrative data on targeting costs was not collected as part of the TUP program, so we turn to other studies of program targeting to estimate the costs of CBT and asset-based (or PMT) methods. We treat the costs of an asset index-based and PMT approach as equivalent in this section, as they both require comprehensive household surveys.\footnote{In practice, an asset-based approach may be slightly cheaper than a PMT, as it does not require conducting a consumption module for a subset of surveys to train a PMT.} We identify three studies that provide variable targeting costs for PMT and CBT methods: \cite{alatas2012} provide variable costs for CBT and PMT-based targeting of a single program in Indonesia; \cite{karlan2013} provide variable costs for CBT and PMT-based targeting of an ultra-poor program in Honduras and one in Peru; and \cite{schnitzer2021targeting} provide variable costs for three CBT-based programs and four PMT-based programs in seven countries in Sub-Saharan Africa.\footnote{To our knowledge, no studies incorporate fixed targeting costs, as these are typically indistinguishable from fixed costs of other components of program set-up.} Table \ref{appendix:costliterature} summarizes the cost estimates from each of these papers; we use the median per-household targeting cost for each method in our analysis (\$2.20 per household for CBT and \$4.00 per household for PMT). While using these global estimates to inform our model of targeting costs in Afghanistan is not ideal, since no data on targeting costs from the TUP program or other anti-poverty programs is available for the country, these values are the best available estimate on which to base our cost analysis. 

We are unable to find any papers that document the targeting cost associated with consumption-based targeting, as consumption data is rarely used as a real-world targeting strategy. We therefore consider the costs of consumption to be strictly greater than the costs of targeting on a PMT, since consumption modules take longer to collect than PMT data in household surveys. In practice, we expect that the cost of targeting on consumption would be substantially greater than the cost of targeting on a PMT.

For phone-based targeting, we associate no cost with the collection and analysis of phone data. While in some cases phone data may require purchase from the operator, partnerships between mobile network operators and governments for social protection and public health applications have not, to date, involved payment \citep{milusheva2021challenges}. The fixed cost of mobile data analysis is non-negligible but its contribution to marginal cost is close to zero as the number of screened households increases. A phone-based targeting method that collects informed consent from program applicants to analyze phone data would have nonzero marginal costs, though the cost of consent would depend on the modality of consent collection. If consent was collected in person, these costs would likely be only slightly lower than those of a PMT, as every household would need to be surveyed in person. If consent was collected over the phone via SMS or voice, these costs would likely  be significantly lower.  

It is worth noting that our benchmark in this paper is the hybrid model with a CBT plus verification component, but due to limited estimates in the literature we leave this strategy out of our cost analysis. We consider the CBT a lower-bound estimate for the hybrid strategy, and therefore our results would be qualitatively unchanged if the hybrid strategy were also considered in cost comparison. \cite{alatas2012} suggest that there are synergies in targeting approaches so that combining approaches is less costly than the sum of the costs of the two approaches individually, but costs are certainly greater than that of CBT targeting alone.  

Our cost analysis finally relies upon administrative data from the TUP program. The TUP program in its entirety served 7,500 households across six provinces of Afghanistan. While there is no data available on the total number of households screened by the TUP program, the portion of the program in Balkh province that was enrolled in the RCT identified 1,235 ultra-poor households out of 20,702 households screened \citep{bedoya2019}. Assuming similar eligibility rates across Afghanistan, we estimate that the TUP program as a whole likely screened around 125,721 households. We use this value to estimate total targeting costs for the TUP program under counterfactual targeting approaches. Eligible households received benefits totaling \$1,688, including a productive asset, cash transfers, a health voucher, training, biweekly social worker visits, and veterinarian visit once every two months during the year of intervention. The total benefits dispersed by the program were therefore on the order of 12.7 million (although the total program costs, including overhead, were closer to 15 million \citep{bedoya2019}); we use the total value of benefits to compare the costs of program targeting using our set of counterfactual targeting approaches to the direct costs of program benefits in Table \ref{appendix:costs}. We find that targeting costs for a PMT or asset-based approach would represent approximately 3.97\% of the total benefits delivered in the program; costs for a CBT approach would represent approximately 2.18\% of the total benefits. In comparison, costs for the phone-based approach would be negligible.

When it comes to speed, in-person data collection for an asset-based (or PMT) targeting approach typically takes months or years to prepare and implement \citep{WorldBank_2020}. The CDR-based approach can be rolled out comparatively quickly --- but there are still practical hurdles to implementation. First, training data for the CDR-based poverty prediction model must be collected, preferably shortly prior to program roll-out \citep{aiken_machine_2021}. While in the TUP project training data was collected in-person in a household survey, in other contexts training data collection was expedited via a phone survey \citep{blumenstock2015, aiken_machine_2021}. Even if data is collected over the phone, it will typically take several weeks to design a survey instrument and collect data. Second, the CDR-based method requires data from mobile network operators. Data sharing agreements with mobile network operators take at minimum a few weeks to arrange, and substantially longer in the worst case \citep{milusheva2021challenges}. Third, and finally, training a CDR-based poverty prediction model is expensive in terms of memory,  computing power, and human capacity, and will likely take several weeks to implement. 



\pagebreak
\section*{Supplementary Tables and Figures}
\label{appendix:supplementaryfigures}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% FIGURES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{figure}[H]
    \centering
    \includegraphics[width=1\textwidth]{appendix_assets.png}
    \caption{Histograms showing the distribution of each underlying asset used to construct the asset index.}
    \label{appendix:assetindex}
\end{figure}


\begin{figure}[H]
    \centering
    \includegraphics[width=1\textwidth]{appendix_kde_outcomes.png}
    \caption{Distributions of asset index and log-transformed consumption, for the entire survey sample, separately for ultra-poor and non-ultra-poor households, and again separately for households in the subsample matched to CDR, households outside of the matched subsample that report owning at least one mobile phone, and households outside of the matched subsample that report not owning a mobile phone.}
    \label{appendix:kdeoutcomes}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=1\textwidth]{appendix_correlations.png}
    \caption{Correlation between asset index and log-transformed consumption, separately for the entire survey sample and the matched subsample. We include the LOESS fit, along with a 95\% confidence interval.}
    \label{appendix:correlations}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=1\textwidth]{tables/appendix_feature_kdes.png}
    \caption{Kernel density estimates for 16 of the most important features for predicting ultra-poor status from CDR, with density estimates shown separately from UP and NUP households. Since many features are near-redundant, rather than showing the raw top 16 features from the table above, we show 16 selected features from the top 50.  See Appendix \ref{appendix:abbreviations} for abbreviations in feature names.}
    \label{appendix:feature_kdes}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TABLES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\clearpage
\pagebreak


\input{tables/appendix_first_component}
\pagebreak

\input{tables/appendix_importances}
\pagebreak

\input{tables/appendix_ml_details}
\input{tables/appendix_asset_based_prediction}
\pagebreak


\input{tables/appendix_combined}

\input{tables/appendix_onesplit}

\input{tables/appendix_individual}

\input{tables/appendix_ml_results}

\input{tables/appendix_costs}

\input{tables/appendix_cost_literature}

\pagebreak


%\input{tables/appendix_consumption}


==> Targeting Paper_COPY2/tables/balance_of_covariates.tex <==
\begin{table}[htb] \centering 
  \caption{Summary statistics for different samples of survey respondents\label{selectionintosample}}
\renewcommand{\arraystretch}{1.2}
\begin{threeparttable}
\begin{footnotesize}
\begin{tabular}{lcccc}
\toprule
 & (1) & (2) & (3) & (4) \\
  \textbf{Outcome}  & \textbf{Full sample} & \textbf{Matched} & \textbf{Unmatched} & \textbf{Unmatched} \\
                                    & \textbf{(all observations)} & \textbf{Subsample} & \textbf{Owns Phone} & \textbf{No Phone} \\ 
\midrule 
\\ [-0.8em]
\multicolumn{5}{l}{\textit{Panel A: Balance of Covariates}} \\ 
[0.3em]
                        Ultra-Poor &      0.42 (0.49) &       0.27 (0.45) &            0.40 (0.49) &         0.66 (0.47) \\
                       Asset Index &      0.00 (2.01) &       1.36 (2.60) &           -0.05 (1.76) &        -1.35 (0.79) \\
                  Log Expenditures &      4.43 (0.71) &       4.64 (0.70) &            4.46 (0.70) &         4.12 (0.65) \\
                          \# Phones &      1.35 (1.18) &       1.72 (1.33) &            1.59 (1.04) &         0.00 (0.00) \\
               Food Security Index &      0.30 (0.90) &       0.35 (0.74) &            0.34 (0.93) &         0.10 (0.89) \\
         Financial Inclusion Index &      0.15 (1.27) &       0.34 (1.39) &            0.15 (1.32) &        -0.05 (0.79) \\
    Psychological Well-being Index &      0.35 (1.01) &       0.38 (1.00) &            0.43 (0.97) &        -0.02 (1.07) \\
                         CWR Group &      0.62 (0.90) &       0.89 (1.02) &            0.62 (0.88) &         0.26 (0.66) \\
\\ [-0.5em]
\multicolumn{5}{l}{\textit{Panel B: Correlations Between Outcomes}} \\
[0.3em]
       Ultra-Poor $\longleftrightarrow$ Asset Index &            -0.32 &             -0.30 &                  -0.27 &               -0.14 \\
  Ultra-Poor $\longleftrightarrow$ Consumption &            -0.39 &             -0.30 &                  -0.39 &               -0.26 \\
 Asset Index $\longleftrightarrow$ Consumption &             0.37 &              0.34 &                   0.34 &                0.15 \\ 
 \\[-0.9em]
                                 $N$ &             2,814 &               535 &                   1,807 &                 472 \\
\bottomrule
 \\[-2.5ex] 
\end{tabular} 
\end{footnotesize}
\begin{tablenotes}[normal,flushleft]
\footnotesize
\item \emph{Notes}: Table reports average characteristics, with standard deviations in parentheses, of TUP survey respondents. Each column represents a different sample of respondents: (1) all respondents in the TUP survey; (2) Just those respondents who own a phone, where the phone number matches to the CDR obtained from the mobile phone operator; (3) Respondents who report owning a phone, but whose phone number does not match to the CDR obtained from the operator; (4) Respondents who report they do not own a phone.
\end{tablenotes}
\end{threeparttable}
\end{table} 

==> Targeting Paper_COPY2/tables/covariates_classifications.tex <==
\begin{table}[H] \centering 
  \caption{What types of households are misclassified? \label{tp_vs_fn}}
\renewcommand{\arraystretch}{1.2}
\begin{threeparttable}
\begin{footnotesize}
\begin{tabular}{p{3cm}p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}}
\toprule
\multicolumn{10}{l}{\emph{Panel A: Ultra-Poor Households (Differences Between True Positives and False Negatives)}} \\ [.5em]

& \multicolumn{3}{c}{\textbf{Asset Index}} & \multicolumn{3}{c}{\textbf{Consumption}} & \multicolumn{3}{c}{\textbf{CDR}} \\

& \textbf{TP} &  \textbf{FN} &  \textbf{Diff.} & \textbf{TP} &  \textbf{FN} &  \textbf{Diff.} & \textbf{TP} &  \textbf{FN} &  \textbf{Diff.} \\
\cmidrule{2-10}
      Ultra-Poor &   1.00 (0.00) &   1.00 (0.00) &   0.00 (0.00) &   1.00 (0.00) &   1.00 (0.00) &   0.00 (0.00) &   1.00 (0.00) &   1.00 (0.00) &   0.00 (0.00) \\
                   Asset Index &  -1.03 (0.49) &   1.18 (1.34) &  -2.21 (0.17) &  -0.34 (1.09) &   0.47 (1.69) &  -0.81 (0.23) &  -0.09 (1.16) &   0.25 (1.70) &  -0.34 (0.24) \\
              Consumption &   4.21 (0.70) &   4.40 (0.62) &  -0.19 (0.11) &   3.78 (0.32) &   4.74 (0.56) &  -0.96 (0.07) &   4.29 (0.60) &   4.32 (0.71) &  -0.02 (0.11) \\
                      \# Phones &   0.89 (0.68) &   1.63 (1.12) &  -0.74 (0.15) &   1.02 (0.73) &   1.48 (1.14) &  -0.46 (0.16) &   1.18 (0.61) &   1.33 (1.21) &  -0.16 (0.15) \\
           Food Security Index &  -0.59 (1.13) &  -0.51 (1.10) &  -0.08 (0.18) &  -0.83 (1.19) &  -0.32 (0.99) &  -0.51 (0.18) &  -0.51 (1.14) &  -0.58 (1.09) &   0.07 (0.19) \\
     Financial Inclusion Index &  -0.00 (0.79) &   0.29 (1.02) &  -0.29 (0.15) &   0.10 (0.80) &   0.19 (1.02) &  -0.09 (0.15) &   0.16 (0.98) &   0.14 (0.88) &   0.02 (0.16) \\
 Psychological Wellbeing Index &  -0.35 (0.92) &  -0.13 (0.94) &  -0.22 (0.15) &  -0.37 (0.86) &  -0.12 (0.98) &  -0.24 (0.15) &  -0.31 (0.81) &  -0.17 (1.02) &  -0.14 (0.15) \\
                     CWR Group &   0.09 (0.44) &   0.01 (0.12) &   0.07 (0.05) &   0.02 (0.12) &   0.08 (0.41) &  -0.06 (0.05) &   0.06 (0.40) &   0.04 (0.24) &   0.03 (0.06) \\[1.2em]
\midrule
\\[-.5em]
\multicolumn{10}{l}{\emph{Panel B: Non-Ultra-Poor Households (Differences Between True Negatives and False Positives)}}\\[.5em]

& \multicolumn{3}{c}{\textbf{Asset Index}} & \multicolumn{3}{c}{\textbf{Consumption}} & \multicolumn{3}{c}{\textbf{CDR}} \\

& \textbf{TN} &  \textbf{FP} &  \textbf{Diff.} & \textbf{TN} &  \textbf{FP} &  \textbf{Diff.} & \textbf{TN} &  \textbf{FP} &  \textbf{Diff.} \\
\cmidrule{2-10}
Ultra-Poor &   0.00 (0.00) &   0.00 (0.00) &   0.00 (0.00) &   0.00 (0.00) &   0.00 (0.00) &   0.00 (0.00) &   0.00 (0.00) &   0.00 (0.00) &   0.00 (0.00) \\
                   Asset Index &   2.53 (2.62) &  -1.08 (0.50) &   3.61 (0.16) &   2.06 (2.92) &   0.94 (1.75) &   1.12 (0.26) &   1.94 (2.87) &   1.43 (2.27) &   0.51 (0.30) \\
              Consumption &   4.82 (0.66) &   4.57 (0.65) &   0.25 (0.08) &   4.97 (0.58) &   3.98 (0.23) &   0.99 (0.04) &   4.78 (0.68) &   4.74 (0.61) &   0.04 (0.08) \\
                      \# Phones &   2.11 (1.43) &   0.96 (0.76) &   1.15 (0.12) &   1.98 (1.49) &   1.52 (0.92) &   0.46 (0.13) &   1.91 (1.44) &   1.80 (1.24) &   0.11 (0.16) \\
           Food Security Index &   0.24 (0.87) &  -0.16 (1.03) &   0.40 (0.13) &   0.24 (0.88) &  -0.14 (0.99) &   0.37 (0.12) &   0.15 (0.91) &   0.18 (0.94) &  -0.02 (0.12) \\
     Financial Inclusion Index &   0.80 (4.92) &  -0.01 (0.82) &   0.82 (0.29) &   0.77 (4.94) &   0.18 (1.24) &   0.59 (0.31) &   0.78 (4.98) &   0.17 (1.10) &   0.61 (0.31) \\
 Psychological Wellbeing Index &   0.69 (0.97) &   0.21 (0.75) &   0.47 (0.10) &   0.62 (0.98) &   0.49 (0.80) &   0.13 (0.11) &   0.62 (0.95) &   0.49 (0.93) &   0.13 (0.12) \\
                     CWR Group &   1.30 (1.00) &   0.84 (0.96) &   0.46 (0.12) &   1.23 (1.03) &   1.13 (0.94) &   0.10 (0.12) &   1.26 (1.01) &   1.01 (0.98) &   0.25 (0.12) \\
\bottomrule
 \\[-2.5ex] 
\end{tabular} 
\end{footnotesize}
\begin{tablenotes}[normal,flushleft]
\footnotesize
\item \emph{Notes}: Table shows the average characteristics (with standard deviations in parentheses) of households that are correctly classified (True Positives [TP] and True Negatives [TN]) and incorrectly classified (False Negatives [FN] and False Positives [FP]), as well as the difference in average characteristics between correctly and incorrectly classified households (Diff.).  Panel A: Differences between ultra-poor households correctly classified as such and those misclassified as non-ultra-poor (errors of exclusion). Panel B: Differences between non-ultra-poor households correctly classified as such and those misclassified as ultra-poor (errors of inclusion).
\end{tablenotes}
\end{threeparttable}
\end{table} 

==> Targeting Paper_COPY2/tables/overlap_classifications.tex <==
\begin{table}[H] \centering 
  \caption{Overlap in targeting errors between methods\label{mistakesoverlapexclusion}}
\renewcommand{\arraystretch}{1.2}
\begin{threeparttable}
\begin{footnotesize}
\begin{tabular}{lcccc}
\toprule
                  & \textbf{Asset Index} & \textbf{Consumption} &      \textbf{CDR} & \textbf{Combined} \\
\midrule
\\ [-.9em]
\multicolumn{5}{l}{\emph{Panel A: Overlap in Errors of Exclusion}} \\
      Asset Index &     100.00\% &           65.33\% &   57.33\% &   66.67\% \\
Consumption &      61.25\% &          100.00\% &   56.25\% &   62.50\% \\
              CDR &      51.19\% &           53.57\% &  100.00\% &   63.10\% \\
         Combined &      75.76\% &           75.76\% &   80.30\% &  100.00\% \\
\\[-.8em]
\multicolumn{5}{l}{\emph{Panel B: Overlap in Errors of Inclusion}} \\
      Asset Index &     100.00\% &           26.67\% &   22.67\% &   48.00\% \\
Consumption &      25.00\% &          100.00\% &   16.25\% &   37.50\% \\
              CDR &      20.24\% &           15.48\% &  100.00\% &   46.43\% \\
         Combined &      54.55\% &           45.45\% &   59.09\% &  100.00\% \\
\bottomrule
 \\[-2.5ex] 
\end{tabular} 
\end{footnotesize}
\begin{tablenotes}[normal,flushleft]
\footnotesize
\item \emph{Notes}: Table measures the extent to which the targeting errors produced by each pair of targeting methods overlap. Evaluation is performed on the matched sample of 535 TUP respondents. Panel A: Overlap between ultra-poor households that are misclassified as non-ultra-poor (errors of exclusion) for each targeting method. Panel B: Overlap between non-ultra-poor households that are misclassified as ultra-poor (errors of inclusion).
\end{tablenotes}
\end{threeparttable}
\end{table} 

==> Targeting Paper_COPY2/tables/resultstable.tex <==
\begin{table}[H] \centering 
  \caption{Targeting simulation results\label{resultstable}}
\renewcommand{\arraystretch}{1.2}
\begin{threeparttable}
\begin{footnotesize}
\begin{tabular}{lcccc}
\toprule
 & (1) & (2) & (3) & (4) \\
 \textbf{Targeting Method} &
 \multicolumn{1}{c}{\textbf{AUC}} & 
 \multicolumn{1}{c}{\textbf{Accuracy}} & 
 \multicolumn{1}{c}{\textbf{Precision}} & 
 \multicolumn{1}{c}{\textbf{Recall}} \\
\midrule
\\[-.8em]
\multicolumn{5}{l}{\emph{Panel A: Matched Sample (N=535) - for whom we have survey and CDR data}} \\[0.3em]
                              Random &  0.50 (0.028) &  0.60 (0.025) &  0.27 (0.038) &  0.27 (0.038) \\
                           Asset Index &  0.73 (0.024) &  0.72 (0.020) &  0.49 (0.041) &  0.49 (0.041) \\
                      Consumption &  0.71 (0.026) &  0.69 (0.023) &  0.45 (0.038) &  0.45 (0.038) \\
                                   CDR &  0.68 (0.027) &  0.69 (0.021) &  0.42 (0.042) &  0.42 (0.042) \\
                              Combined &  0.78 (0.022) &  0.75 (0.020) &  0.55 (0.039) &  0.55 (0.039) \\
                              
                              
%\midrule
\\ [-0.8em]
\multicolumn{5}{l}{\emph{Panel B: Balanced Sample (N=1,007) - as above, plus households without phones}} \\[0.3em]
                              Random &  0.50 (0.017) &  0.90 (0.006) &  0.05 (0.010) &  0.05 (0.010) \\
                           Asset Index &  0.72 (0.026) &  0.90 (0.006) &  0.10 (0.013) &  0.10 (0.013) \\
                      Consumption &  0.70 (0.028) &  0.90 (0.006) &  0.15 (0.025) &  0.15 (0.025) \\
                                CDR (Target Phoneless First) &  0.68 (0.030) &  0.90 (0.006) &  0.11 (0.035) &  0.11 (0.035) \\
           CDR (Target Phoneless Last) &  0.51 (0.028) &  0.90 (0.006) &  0.12 (0.033) &  0.12 (0.033) \\

               Combined (Target Phoneless First) &  0.74 (0.026) &  0.90 (0.006) &  0.11 (0.046) &  0.11 (0.046) \\
      Combined (Target Phoneless Last) &  0.57 (0.022) &  0.90 (0.006) &  0.18 (0.007) &  0.18 (0.007) \\
%\midrule
\\[-0.8em]
\multicolumn{5}{l}{\emph{Panel C: Full Sample (N=2,814) - as above, plus households with phones on other networks}} \\[0.3em]
                              Random &  0.50 (0.009) &  0.89 (0.005) &  0.06 (0.007) &  0.06 (0.007) \\
                           Asset Index &  0.65 (0.017) &  0.89 (0.005) &  0.07 (0.014) &  0.07 (0.014) \\
                      Consumption &  0.69 (0.015) &  0.89 (0.006) &  0.08 (0.031) &  0.08 (0.031) \\
                                CDR (Target Phoneless First) &  0.52 (0.008) &  0.89 (0.005) &  0.06 (0.008) &  0.06 (0.008) \\
           CDR (Target Phoneless Last) &  0.48 (0.008) &  0.89 (0.005) &  0.08 (0.010) &  0.08 (0.010) \\

               Combined (Target Phoneless First) &  0.52 (0.008) &  0.89 (0.005) &  0.06 (0.008) &  0.06 (0.008) \\
      Combined (Target Phoneless Last) &  0.49 (0.008) &  0.89 (0.005) &  0.09 (0.009) &  0.09 (0.009) \\
\bottomrule
 \\[-2.5ex] 
\end{tabular} 
\end{footnotesize}
\begin{tablenotes}[normal,flushleft]
\footnotesize
\item \emph{Notes}: Four different measures of performance (columns) reported for different targeting methods (rows), using different samples of survey respondents (panels). Standard deviations, calculated using 1,000 bootstrap samples, in parentheses. Panel A: The 535-household subsample that is matched to CDR. Panel B: The 535-household matched sample, plus the 472 households that do not have a phone; this is meant to approximate targeting performance if CDR from all mobile networks were available. Sample weights are applied as described in Section \ref{section:evaluation}. Panel C: All 2,814 observations from the TUP survey, including households matched to CDR, households that own phones not matched to CDR, and households without phones, with sample weights applied. For Panels B and C, we simulate two types of CDR-based targeting: targeting households without phones first and targeting households without phones last. 
\end{tablenotes}
\end{threeparttable}
\end{table} 


==> intro_new.tex <==
% TODO

% Defining who is eligible for specific aid programs---targeting---has far-reaching economic and social implications. However, targeting can be costly, and often introduces significant errors of inclusion and exclusion \citep{alatas2012, alatas2016, brown2018, coady2004}. Finding cost-effective approaches to minimize targeting errors has become increasingly important within the global context of rapidly expanded social protection programs and increasing government debt. The visibility and importance of aid and aid targeting has increased dramatically in the past year: In 2020, global extreme poverty increased for the first time in two decades - driven by the COVID-19 pandemic, and exacerbated by the effects of conflict and climate change \citep{WorldBank_2020}. Most countries temporarily expanded their social protection programs in response to the pandemic, with more than 1.1 billion new recipients receiving government-led social assistance payments \citep{Gentilini2020}. 

% In high-income countries, targeting frequently relies on administrative data such as tax records or comprehensive social registries of poverty using metrics such as income or consumption. Low- and middle-income countries (LMICs), characterized by high levels of informality and a dearth of verifiable income data, typically follow alternative strategies that rely on primary data collection. However, feasibility of primary data collection and the reliability of these data are likely to introduce significant errors in the targeting process \citep{Deaton2016,jerven, wb_forthcoming}. These issues are exacerbated in fragile and conflict-affected countries, where two thirds of the world's poor are expected to reside by 2030 \citep{corral2020}. 


Recent studies have shown that non-traditional ``digital trace'' data---behavioral indicators recorded in everyday interactions with technology---are predictive of wealth in LMIC contexts \citep[e.g.][]{blumenstock2015, ermon2019}. There is optimism in the machine learning and development communities that these data could provide a quick and low-cost alternative or complement to standard field-based targeting methods, helping overcome logistical constraints to data collection, and increasing the cost-effectiveness of targeting  \citep[e.g.][]{blumenstock2016, dearteaga2018}.


In high-income countries, poverty targeting frequently relies on means-based testing, restricting program benefits to those below a certain income threshold based on administrative data such as tax records. In LMICs, means tests are often impractical due to high levels of informality. Traditional approaches in these countries rely on geographic targeting or proxy measures of economic well-being such as proxy-means testing (PMT), community-based targeting or a combination of these methods. PMTs use data on assets and demographic characteristics to create a proxy for consumption or income, while community-based methods allow community members and leaders to participate in the identification of eligible aid recipients. These approaches are imperfect, and inevitably lead to significant targeting errors; however, \cite{hannaolken} provide empirical evidence that narrowly-targeted programs can be significantly more cost-effective than widely-targeted programs or universal allocation, even when targeting is based on imperfect poverty proxies. 


Motivated by the importance of targeting for efficient allocation of development aid, a significant body of research has explored ways to improve targeting accuracy. 
A meta-analysis including 8 PMTs and 14 community-based targeting strategies finds that a similar level of resources went to the poorest 40\% in both community-based and PMT-based targeting methods \citep{coady2004}. Similarly, recent experimental evidence finds that differences in targeting errors across PMT, community-based and hybrid methods in Indonesia, India, Mali, Peru, Honduras and Niger, are often small relative to the base level of targeting errors using different benchmarks of well-being \citep{alatas2012,banerjee2007,Fortinetal2016,karlan2013,Premandetal2020}.\footnote{\citep{coady2004} find that targeting turned out to be regressive in a quarter of programs reviewed. This highlights the inherent challenges with measurement. Consumption and poverty estimates are based on surveys with quality issues, and ``in some cases, the problems are severe enough to threaten even the most basic understanding of growth, poverty and inequality" \citep{Deaton2016}.}
  
While \textit{per capita} consumption is often used as a benchmark to estimate poverty and measure targeting errors, the evidence comparing PMT and community-based approaches suggests that communities may apply a broader concept of poverty---for instance, including factors that predict earnings capacity. Community-based methods also typically yield higher rates of community satisfaction levels than PMT methods, when elite capture is absent. \citep{alatas2012,banerjee2007,Fortinetal2016,karlan2013,Premandetal2020}.\footnote{Contrary to this evidence, a study in Cameroon finds that community-based targeting methods performed consistently worse compared to PMT selection when assessed against consumption. However, the authors explained, that these are in part driven by communities including human and physical capital asset holding in the selection criteria---consistent with a multidimensional concept of poverty---and also due to implementation issues, reflected in errors of exclusion and inclusion above 40\% for PMT \citep{Stoeffler2016}}. While the idea that poverty is multidimensional is now well-established, how to apply these ideas to the assessment of targeting accuracy remains a challenge \citep{Alkire2015,Sen2010}. In this paper, we consider the hybrid approach selected by the government as the benchmark for capturing multidimensional poverty on which alternative targeting methods are compared against.  

Regardless of their accuracy (or inaccuracy), the current methods available for poverty targeting in LMICs are time- and resource-intensive, and  may be infeasible in fragile or conflict-affected areas or in contexts when mobility and social interaction is limited, such as during the current pandemic. We turn, therefore, to the literature on using passively collected digital trace data to estimate wealth, and later evaluate whether methods based on these data are useful for identifying the poor and the very poor. 



\subsubsection{Wealth Estimation from Mobile Phone Metadata}

Research to date on wealth prediction from digital trace data has focused on mobile phone metadata as cell phones have become increasingly ubiquitous worldwide, projected to reach a global penetration rate of 70\% in 2025 \citep{gsma}. Recent work has shown that machine learning methods leveraging CDR can produce useful estimates of wealth and well-being at a fine spatial granularity. This body of work focuses largely on poverty, typically quantified by an asset-based wealth index \citep[e.g.][]{blumenstock2015, hernandez}, but related papers explore a wider set of well-being measures, including literacy \citep{schmid}, food security \citep{decuyper1}, and infrastructure \citep{blumenstock2017}.

While most of this work addresses spatially granular poverty mapping, to our knowledge two papers to date cover the individual-level wealth prediction task that is more relevant to poverty targeting. \cite{blumenstock2015} show that CDR data are predictive of an individual-level asset-based wealth index in Rwanda. More specifically, the study matches ground-truth survey data to call detail records covering two years of mobile phone activity for 856 geographically stratified individuals, extracts a suite of thousands of behavioral indicators from the CDR covering different aspects of mobile phone use, and applies a supervised learning algorithm to generate wealth predictions from behavioral indicators. Model accuracy is evaluated with cross-validation to ensure that the wealth prediction model generalizes out-of-sample (cross-validated $r$ = 0.68). \cite{blumenstock2018} performs the same experiment for 1,234 male heads of households in the Kabul and Parwan districts of Afghanistan, yielding similar predictive accuracy.

\subsection{Our Contribution}

Given the success of wealth prediction from mobile phone data and the need for cheaper and more accurate targeting mechanisms in the LMICs, exploring poverty targeting based on CDR methods presents a natural extension of the existing literature. Here we build on the evidence on poverty targeting and wealth prediction from digital trace data to evaluate whether CDR data can be used in practice to target the very poor for anti-poverty programs. By matching CDR to household survey data from 535 households in 80 of the poorest villages in the Balkh province of Afghanistan, we assess whether CDR-based methods can replicate household-level targeting using a hybrid method from a recent program intended for ultra-poor households. We find that CDR-based targeting is as accurate as targeting based on assets or consumption for the subset of households that own a mobile phone in this sample, and that targeting based on a combination of assets, consumption, and CDR data is more accurate than targeting based on any one method assessed. We also analyze options for targeting the non-phone-owning ultra-poor household under CDR-based targeting regimes, noting in particular that allocating benefits to all non-phone-owning households does not compromise the accuracy of CDR-based targeting.%
\footnote{JB add reference to \citet{aiken_machine_2021}.}
We conclude by discussing the important ethical and logistical considerations that may influence how CDR methods are used to support targeting efforts in practice.


